How Nonconformity Functions and Difficulty of Datasets Impact the Efficiency of Conformal Classifiers

The property of conformal predictors to guarantee the required accuracy rate makes this framework attractive in various practical applications. However, this property is achieved at a price of reduction in precision. In the case of conformal classification, the systems can output multiple class labels instead of one. It is also known from the literature, that the choice of nonconformity function has a major impact on the efficiency of conformal classifiers. Recently, it was shown that different model-agnostic nonconformity functions result in conformal classifiers with different characteristics. For a Neural Network-based conformal classifier, the inverse probability (or hinge loss) allows minimizing the average number of predicted labels, and margin results in a larger fraction of singleton predictions. In this work, we aim to further extend this study. We perform an experimental evaluation using 8 different classification algorithms and discuss when the previously observed relationship holds or not. Additionally, we propose a successful method to combine the properties of these two nonconformity functions. The experimental evaluation is done using 11 real and 5 synthetic datasets.

==> makejmlrbook <==
#!/usr/bin/env perl
# File          : makejmlrbook
# Author        : Nicola L C Talbot
# Date          : 22nd March 2010
# Last Modified : 21st September 2020
# Version       : 0.33
# Description   : Given the name of a document using the
#                 jmlrbook class file, this script runs
#                 pdflatex (and possibly bibtex) on the
#                 imported articles and the main document.
# http://www.dickimaw-books.com/
#
# This file is distributed as part of the jmlr LaTeX bundle.
#
# *****
# This script is now obsolete and will be removed in later
# distributions. Use MakeJmlrBookGUI instead:
# https://www.dickimaw-books.com/software/makejmlrbookgui
# *****
#
# Copyright (c) 2006-2020 Nicola L.C. Talbot
# This work may be distributed and/or modified under the
# conditions of the LaTeX Project Public License, either version 1.3
# of this license or any later version.
# The latest version of this license is in
#   http://www.latex-project.org/lppl.txt
# and version 1.3 or later is part of all distributions of LaTeX
# version 2005/12/01 or later.
#
# This work has the LPPL maintenance status `maintained'.
#
# The Current Maintainer of this work is Nicola Talbot.

use Getopt::Long;
use File::Basename;
use File::Copy;
use Cwd;
use strict;

my $version = "0.33 (2020-09-21)";

my $eol = "\n";
my $dd  = '/';

if ($^O eq 'MSWin32')
{
  $eol = "\r\n";
  $dd = "\\";
}

my $showversion      = 0;
my $showhelp         = 0;
my $quiet            = 0;
my $batchtex         = 0;
my $online           = 1;
my $print            = 1;
my $html             = 1;
my $latexapp         = 'pdflatex';
my $bibtexapp        = 'bibtex';
my $latexopts        = '';
my $bibtexopts       = '';
my $format           = 'pdf';
my $logourl          = '';
my $extractpreface   = 0; # v0.3 added
# execute system calls (--noexecute will just list the system calls
# without executing them)
my $execute          = 1; # v0.31 added

my $appname = basename($0);

warn <<__END_OBSOLETE_WARN;
Warning: $appname is now obsolete and will be removed in later
distributions. Use MakeJmlrBookGUI instead:
https://www.dickimaw-books.com/software/makejmlrbookgui

__END_OBSOLETE_WARN

unless(&GetOptions(
   "online!"          => \$online,
   "print!"           => \$print,
   "html!"            => \$html,
   "extractpreface!"  => \$extractpreface,
   "logourl=s"        => \$logourl,
   "format=s"         => \$format,
   "latexapp=s"       => \$latexapp,
   "bibtexapp=s"      => \$bibtexapp,
   "latexopts=s"      => \$latexopts,
   "bibtexopts=s"     => \$bibtexopts,
   "quieter!"         => \$quiet,
   "batchtex!"        => \$batchtex,
   "execute!"         => \$execute,
   "version"          => \$showversion,
   "help"             => \$showhelp))
{
   die "Use --help for help\n";
}

if ($showhelp)
{
  die "$appname version $version Copyright (c) 2010 Nicola L C Talbot\n",
    "Distributed under the LaTeX Project Public License.\n\n",
    "Syntax: $appname [options] <filename>\n\n",
    "<filename> should be the name of the master document for a LaTeX \n",
    "file that uses the jmlrbook class. The .tex extension may be\n",
    "omitted.\n\n",
    "Basic options:\n",
    "--online\t\tGenerate the color on-line version (default)\n",
    "--noonline\t\tDon't generate the color on-line version\n",
    "--print\t\t\tGenerate the grayscale print version (default)\n",
    "--noprint\t\tDon't generate the grayscale print version\n",
    "--html\t\t\tGenerate the HTML version (default)\n",
    "--nohtml\t\tDon't generate the HTML version\n",
    "--extractpreface\tParse document for preface environment\n",
    "--noextractpreface\tDon't parse document for preface environment\n",
    "--logourl <url>\tMake the logo on the HTML index page link to <url>\n",
    "--batchtex\t\tRun TeX in batch mode\n",
    "--nobatchtex\t\tDon't run TeX in batch mode\n",
    "--quieter\t\tReduce messages to stdout and run TeX in batch mode\n",
    "--noquieter\t\tDon't reduce messages to stdout\n",
    "--execute\t\tExecute system calls (default)\n",
    "--noexecute\t\tDon't execute system calls, just list the\n",
    "\t\t\tcommands.\n",
    "--version\t\tDisplay version number and exit\n",
    "--help\t\t\tDisplay help message and exit\n",
    "\nAdvanced options:\n",
    "--latexapp <name>\tApplication used to call LaTeX\n",
    "\t\t\t(Defaults to 'pdflatex')\n",
    "--format <string>\tOutput format (default: 'pdf')\n",
    "--bibtexapp <name>\tApplication used to call BibTeX\n",
    "\t\t\t(Defaults to 'bibtex')\n",
    "--latexopt <string>\tOptions to pass to LaTeX\n",
    "--bibtexopt <string>\tOptions to pass to BibTeX\n";
}

if ($showversion)
{
  die "$appname version $version copyright (c) 2010 Nicola L C Talbot\n",
    "Distributed under the LaTeX Project Public License.\n";
}

unless ($#ARGV == 0)
{
   die "$appname: missing filename\n",
       "use --help for help\n";
} 

if ($quiet or $batchtex)
{
   $latexopts = '-interaction=batchmode '.$latexopts;
}

if ($quiet)
{
   $bibtexopts = '-terse '.$bibtexopts;
}

my ($main_name, $main_path, $main_suffix) 
  = fileparse($ARGV[0], '\.(tex|ltx)');

$main_suffix = '.tex' unless $main_suffix;

my $org_dir = cwd();

&chdirordie($main_path);

my $mainaux = "$main_name.aux";

# If the aux file doesn't exist or the aux file is older than
# the main file, run latex

if (not -e $mainaux or (-M $mainaux > -M "$main_name$main_suffix"))
{
   &latex($main_name);
}

my $main_bibdata = 0;
my @imports = ();
my %pagerefs = ();
my $preface_data; # v0.3 new
my @preface_editors = ();

# Parse aux file

&parsemainaux($mainaux);

# Replace any instances of \articlepagesref

foreach my $import (@imports)
{
   my $label = $import->{'label'};

   my $pages = $pagerefs{$label}->{'start'}.'--'
             . $pagerefs{$label}->{'end'};

   $import->{'author'}=~s/\\articlepagesref\s*\{$label\}/$pages/;
}

if ($html)
{
   # If the html files need to be created, make the directory
   # html-src, if it doesn't already exist

   unless (-d 'html-src')
   {
      &mkdirordie('html-src');
   }

   unless (-d 'html')
   {
      &mkdirordie('html');
   }

   if ($extractpreface) # v0.3 new
   {
      # If the preface needs to be extract, make a directory for it if
      # it doesn't already exist

      my $prefdir = &fname("html-src", $preface_data->{'OutFile'});

      unless (-d $prefdir)
      {
         &mkdirordie($prefdir);
      }

      my $prefbase = &fname($prefdir, $preface_data->{'OutFile'});

      &createprefacefile($prefdir, $prefbase);

      # Create the cfg file

      &createjmlrcfg("html-src", $preface_data->{'OutFile'});

      &chdirordie($prefdir);

      &latex($preface_data->{'OutFile'});
      &htlatex($preface_data->{'OutFile'}, 'jmlr');

      &chdirordie($org_dir, $main_path);

      # Check the appropriate subdirectory is in html directory

      my $outname = &fname('html', $preface_data->{'OutFile'});

      unless (-d $outname)
      {
         &mkdirordie($outname);
      }

      # Copy pdf file

      &copyordie("$prefbase.$format",
                &fname($outname, "$preface_data->{OutFile}.$format"));

      # Copy html file

      &copyhtml($preface_data->{'OutFile'}, $preface_data->{'OutFile'});
   }
}

# Iterate through each imported article

foreach my $import (@imports)
{
   my $label = $import->{'label'};
   my $importbase = &fname($import->{'path'}, $import->{'name'});

   # Check the aux file of this article

   my $aux = "$importbase.aux";

   # The aux file should exist because running LaTeX on the
   # main file will create the aux file.

   my $bibdata = 0;

   if (open AUX, $aux)
   {
      &message("Reading '$aux'...\n");

      while (<AUX>)
      {
         if (/\\bibdata\b/)
         {
            $bibdata = 1;
         }
      }
  
      close AUX;
   }
   elsif (not $execute)
   {
      warn "Can't open '$aux' - skipping\n";
   }
   else
   {
      die "$appname: Can't open '$aux' $!\n";
   }

   # Do we need a bibtex run?

   if ($bibdata)
   {
      my $log = "$importbase.log";

      # If the log file doesn't exist, run LaTeX

      unless (-e $log)
      {
         &chdirordie($import->{'path'});

         &latex($import->{'name'});

         &chdirordie($org_dir, $main_path);
      }

      open LOGFD, $log or die "$appname: Can't open '$log' $!\n";

      &message("Reading '$log'...\n");

      my $runbibtex = 0;

      while (<LOGFD>)
      {
         if (/There were undefined citations\./)
         {
            # Run bibtex and latex
            $runbibtex = 1;

            last;
         }
      }

      close LOGFD;

      if ($runbibtex)
      {
         &chdirordie($import->{'path'});

         &bibtex($import->{'name'});
         &latex($import->{'name'});

         &chdirordie($org_dir, $main_path);
      }
   }

   if ($html)
   {
      # If html is required, we also need pdf versions of the
      # individual articles.

      # v0.2 run latex even if pdf file exists to ensure start page 
      # number is correct.

      &chdirordie($import->{'path'});

      &latexstartpage($import->{'name'}, $pagerefs{$label}->{'start'});

      &chdirordie($org_dir, $main_path);

      # Do we need a rerun?

      if (&needs_rerun($importbase))
      {
         &chdirordie($import->{'path'});

         &latexstartpage($import->{'name'}, $pagerefs{$label}->{'start'});

         &chdirordie($org_dir,$main_path);
      }

      my $importdir = $import->{'path'};

      if ($importdir = '.')
      {
         $importdir = $import->{'name'};
      }

      # Check the appropriate subdirectory is in html-src

      my $name = &fname('html-src', $importdir);

      unless (-d $name)
      {
         &mkdirordie($name);
      }

      my $text = '';

      # Read the LaTeX file and store everything up to
      # the end of the abstract

      my $tex = "$importbase.tex";

      my $absfile = &fname("html-src", $importdir,
                           $import->{'name'}.'.tex');

      if ($execute)
      {
         open TEX, $tex or die "$appname: Can't open '$tex': $!\n";

         while (<TEX>)
         {
            # This doesn't handle complicated cases, such as
            # the author using \abstract ... \endabstract
            # or commenting out the abstract with conditionals
            if (/^([^%]*)\\end\{abstract\}/)
            {
               $text .= $&;
               last;
            }

            $text .= $_;
         }

         close TEX;

         # Add the 'html' class option:
         unless ($text=~
          s/^([^%]*)\\documentclass\s*\[(.*)\]/$1\\documentclass[$2,html]/m)
         {
           $text=~s/^([^%]*)\\documentclass\s*/$1\\documentclass[html]/m;
         }

         my $aux = "$importbase.aux";

         $aux=~s/\\/\//g if ($dd eq '\\');

         my $prebegindoc = '\\hypersetup{draft}' . $eol
                         . '\\makeatletter' . $eol
                         . "\\input{../../$aux}" . $eol
                         . '\\makeatother'
                         . $eol;

         my $begindoc = '';

         # Set the authors
         if (defined($import->{'author'}))
         {
            my $author = $import->{'author'};

            $author=~s/^([^;]*);/\\textbf{\\emph{$1};}/;

            $begindoc .= "\\jmlrauthors{$author}";
         }

         # Add content div

         # v0.31 modified \footnote to set the footnote text as in-line
         # parenthesis.

         $text=~s/^([^%\n\r\f]*)\\begin\{document\}/
                 $prebegindoc$&$begindoc
                 \\HCode{<div id="content">}
                 \\renewcommand{\\footnote}[2][]{ (\#2)}%$eol
                 /mx;

         # Create file containing the abstract

         open ABSFD,">$absfile" 
           or die "$appname: Can't create '$absfile': $!\n";

         print ABSFD "\\batchmode", $eol if ($batchtex or $quiet);

         my $texpath = $import->{path};

         $texpath=~s/\\/\//g if ($dd eq '\\');

         print ABSFD
           "\\makeatletter",$eol,
           "\\def\\input\@path{{../../$texpath/}}$eol",
           "\\makeatother",$eol,
           $text, $eol, 
           "\\HCode{", &htmltimestamp, "}", $eol,
           "\\HCode{</div>}", $eol,
           &htmlmenu, # v0.3 added by Olivier Chapelle
           "\\end{document}",$eol;

         close ABSFD;
      }
      else
      {
         &messagecall("Skipping creation of '$absfile'\n");
      }

      # Create the cfg file

      &createjmlrcfg("html-src", $importdir);

      # Run htlatex

      # Change directory
      &chdirordie("html-src", $importdir);

      &htlatex($import->{'name'}, 'jmlr');

      # Go back to main directory

      &chdirordie($org_dir, $main_path);

      # Copy the html file to the html directory, but rename
      # the css file to jmlr.css

      &copyhtml($importdir, $import->{'name'});

      # Check the appropriate subdirectory is in html directory

      my $outname = &fname('html', $importdir);

      unless (-d $outname)
      {
         &mkdirordie($outname);
      }

      # Copy pdf file

      &copyordie("$importbase.$format",
                 &fname($outname, "$import->{name}.$format"));
   }
}

# do we need to run bibtex on the main document?

if ($main_bibdata)
{
   &bibtex($main_name);
}

if ($online)
{
   &latexonline($main_name);

   # do we need a rerun?

   if (&needs_rerun($main_name))
   {
      &message("Rerun required\n");
      &latexonline($main_name);

      # check again

      if (&needs_rerun($main_name))
      {
         &message("Rerun required\n");
         &latexonline($main_name);
      }
   }
}

if ($print)
{
   &latexprint($main_name);

   # do we need a rerun?

   if (&needs_rerun($main_name))
   {
      &message("Rerun required\n");
      &latexprint($main_name);

      # check again

     if (&needs_rerun($main_name))
     {
        &message("Rerun required\n");
        &latexprint($main_name);
     }
   }
}

if ($html and $execute)
{
   # Make the index file

   my $indexfile = &fname('html-src', "index");

   my $preamble = '';

   open OUTFD, ">$indexfile.tex" 
    or die "Can't open '$indexfile.tex': $!\n";

   open INFD, "$main_name.tex"
     or die "Can't open '$main_name.tex': $!\n";

   print OUTFD "\\batchmode", $eol if ($batchtex or $quiet);

   print OUTFD
        "\\makeatletter",$eol,
        "\\def\\input\@path{{../}}$eol",
        "\\makeatother",$eol,
        "\\def\\jmlrgrayscale{0}",$eol;

   while (<INFD>)
   {
      unless
        (s/^([^%]*)\\documentclass\s*\[([^\]]*)\]/
           $1\\documentclass[$2,html]/x)
      {
         s/^([^%]*)\\documentclass\s*/$&\[html\]/;
      }

      s/^([^%]*)\\begin\{document\}/
        \\hypersetup{draft}$eol$&\\HCode{<div id="content">}/x;

      if (/^([^%]*)\\maketitle/)
      {
         $preamble .= join('', $1, "\\maketitle", $eol);
         last;
      }

      $preamble .= $_;
   }

   close INFD;

   # Find the book logo
   if ($preamble
     =~/\\logo\s*(?:\[[^\]]*\])?\s*\{(%\s*\n)?\\includegraphics\s*(\[[^\]]*\])?\{([^}]*)\}\}/m)
   {
      my $texpath = $3;
      my $orgtexpath = $texpath;
      $texpath=~s/\//\\/g if ($dd eq "\\");

      my $ext = '';

      if (-e $texpath)
      {
         &copyordie($texpath, 'html');

         &copyordie($texpath, 'html-src');
      }
      elsif (-e "$texpath.png")
      {
         &copyordie("$texpath.png", 'html');

         &copyordie("$texpath.png", 'html-src');

         $ext = '.png';
      }
      elsif (-e "$texpath.jpg")
      {
         &copyordie("$texpath.jpg", 'html');
         &copyordie("$texpath.jpg", 'html-src');

         $ext = '.jpg';
      }
      elsif (-e "$texpath.gif")
      {
         &copyordie("$texpath.gif", 'html');

         &copyordie("$texpath.gif", 'html-src');

         $ext = '.gif';
      }

      my $img = basename($texpath);
      
      if ($logourl)
      {
         $preamble=~s/
                  \\includegraphics(\[[^\]]*\])?\{$orgtexpath\}/
                  \\href{$logourl}{\\includegraphics${1}{$img$ext}}/mgx;
      }
      else
      {
         $preamble=~s/
                  \\includegraphics(\[[^\]]*\])?\{$orgtexpath\}/
                  \\includegraphics${1}{$img$ext}/mgx;
      }
   }

   print OUTFD $preamble, $eol;

   # Parse TOC

   my $toc = "$main_name.toc";

   # Add link to preface if required

   if ($extractpreface)
   {
      print OUTFD
         "\\begin{description}\\item[\\normalfont \\prefacename]", $eol;

      print OUTFD "\\textbf{\\emph{\\jmlrabbrnamelist{{",
                  join('},{', @preface_editors),
                  "}}};} ",
                  '\\csname @jmlrabbrvproceedings\\endcsname\\space',
                  '\\csname @jmlrvolume\\endcsname:',
                  $preface_data->{'Start'};

      unless ($preface_data->{'Start'} eq $preface_data->{'End'})
      {
         print OUTFD '--', $preface_data->{'End'};
      }

      print OUTFD ', \\csname @jmlryear\\endcsname\\newline', $eol;

      my $name = $preface_data->{'OutFile'};

      print OUTFD "[\\HCode{<a href=\"$name.html\">html</a>}] ",
                  "[\\HCode{<a href=\"$name/$name.pdf\">pdf</a>}]",
                  $eol;

      print OUTFD "\\end{description}$eol";
   }

   open TOC, $toc or die "Can't open '$toc': $!\n";

   my $idx = 0;

   while (<TOC>)
   {
      if (/^\\tocpart\s*\{(.*)\}\s*$/)
      {
         print OUTFD "\\begin{center}\\bfseries $1\\end{center}$eol";
      }
      elsif (/\\contentsline\s*\{papertitle\}\{(.*)\}\{[^{}]*\}\{[^{}]*\}\s*$/)
      {
         # v0.3 Changed by Olivier Chapelle to use description
         # environment instead of paragraph break
         print OUTFD "\\begin{description}\\item[\\normalfont $1]$eol";
      }
      elsif (/\\contentsline\s*\{chapterauthor\}\{(.*)\}\{[^{}]*\}\{[^{}]*\}\s*$/)
      {
         my $details = $1;
         $details=~s/([^;]*);/\\textbf{\\emph{$1};}/;

         my $label = $imports[$idx]->{'label'};
         my $pages = $pagerefs{$label}->{'start'}.'--'
                   . $pagerefs{$label}->{'end'};

         $details=~s/\\articlepagesref\s*\{$label\}/$pages/;

         # v0.3 Changed by Olivier Chapelle to use newline instead of par
         print OUTFD "$details\\newline$eol";

         my $name = $imports[$idx]->{'name'};

         print OUTFD "[\\HCode{<a href=\"$name.html\">abs</a>}] ",
                     "[\\HCode{<a href=\"$name/$name.pdf\">pdf</a>}]",
                     $eol;

         # v0.3 Changed by Olivier Chapelle to end description
         print OUTFD "\\end{description}$eol";

         $idx++;
      }
   }

   close TOC;

   # version 0.2 added time stamp

   print OUTFD "\\HCode{", &htmltimestamp, "}$eol";

   print OUTFD &htmlmenu; # v0.3 Added by Olivier Chapelle

   print OUTFD "\\HCode{</div>}\\end{document}$eol";

   close OUTFD;

   # Go into html-src directory and run htlatex

   &chdirordie('html-src');

   &htlatex("index", 'xhtml');

   &chdirordie('..');

   # Copy to html directory

   my $inname = &fname('html-src', 'index.html');
   my $outname = &fname('html', 'index.html');

   open INFD, $inname or die "Can't open '$inname': $!\n";

   open OUTFD, ">$outname" or die "Can't open '$outname': $!\n";

   while (<INFD>)
   {
      s/href="index.css"/href="jmlr.css"/;

      print OUTFD;
   }

   close OUTFD;

   close INFD;

   # v0.2 new:
   # Copy any images generated by htlatex to html/

   my @imagefiles = glob(&fname('html-src', "index*.png"));

   foreach my $imagefile (@imagefiles)
   {
      copy($imagefile, 'html');
   }
}
elsif ($html)
{
   &messagecall("chdir 'html-src'\n");
   &htlatex("index", 'xhtml');
}

# Return to original directory
chdir $org_dir;

# Subroutines

sub message{ print @_ unless ($quiet) }

sub messagecall{ print @_ if (not $quiet or not $execute) }

sub systemcall{
  my $cmd = shift;

  &messagecall($cmd, "\n");

  my $code = 0;

  $code = system($cmd) if ($execute);

  $code;
}

sub latex{
   my $file = shift;

   my $code = &systemcall(join(' ', $latexapp, $latexopts, "\"$file\""));

   if ($code)
   {
      die "**LaTeX run failed with exit code $code.**\n",
          "Check '$file.log' for details\n";
   }
}

# v0.2 new
sub latexstartpage{
   my $file = shift;
   my $page = shift;

   my $code = &systemcall(join(' ', $latexapp, $latexopts,
     "\"\\def\\startpage{$page}\\input{$file}\""));

   if ($code)
   {
      die "**LaTeX run failed with exit code $code.**\n",
          "Check '$file.log' for details\n";
   }
}

sub copyordie{
   my ($org, $dest) = @_;

   &messagecall("copy '$org' to '$dest'\n");

   if ($execute)
   {
      copy($org, $dest) or die "Can't copy '$org' to '$dest': $!\n";
   }
}

sub latexonline{
   my $file = shift;

   my $code = &systemcall(join(' ', $latexapp, $latexopts,
     "\"\\def\\jmlrgrayscale{0}\\input{$file}\""));

   if ($code)
   {
      die "**LaTeX run failed with exit code $code.**\n",
          "Check '$file.log' for details\n";
   }

   &copyordie("$file.$format", "$file-online.$format");
}

sub latexprint{
   my $file = shift;

   my $code = &systemcall(join(' ', $latexapp, $latexopts,
     "\"\\def\\jmlrgrayscale{1}\\input{$file}\""));

   if ($code)
   {
      die "**LaTeX run failed with exit code $code.**\n",
          "Check '$file.log' for details\n";
   }

   &copyordie("$file.$format", "$file-print.$format");
}

sub bibtex{
   my $file = shift;

   my $code = &systemcall(
                 join(' ', $bibtexapp, $bibtexopts, "\"$file\""));

   if ($code)
   {
      die "**BibTeX run failed with exit code $code.**\n",
          "Check '$file.blg' for details\n";
   }
}

sub needs_rerun{
  my $file = shift;
  my $rerun = 0;

  unless ($execute)
  {
     &messagecall("Skipping rerun check for '$file'\n");
     return 0;
  }

  # Scan log file for rerun message

  my $log = "$file.log";

  # If there's no log file a run is needed
  open LOGFD, $log or return 1;

  while (<LOGFD>)
  {
     if (/Rerun to get cross-references right\./)
     {
        $rerun = 1;
        last;
     }
  }

  close LOGFD;

  return $rerun;
}

sub fname{ join($dd, @_) }

# v0.3 new
sub chdirordie{
  my $dirname = &fname(@_);

  &messagecall("chdir '$dirname'\n");

  unless (chdir $dirname)
  {
     if ($execute)
     {
        die "$appname: Can't change directory to $dirname: $!\n";
     }
     else
     {
        warn "(Can't change directory to '$dirname')\n";
     }
  }
}

# v0.31 new
sub mkdirordie{
  my $dirname = &fname(@_);

  &messagecall("mkdir '$dirname'\n");

  unless (mkdir $dirname)
  {
     if ($execute)
     {
        die "$appname: Can't create directory '$dirname': $!\n";
     }
     else
     {
        warn "(Can't create directory '$dirname')\n";
     }
  }
}

# v0.2 new
sub htmltimestamp{
   my $timestamp = localtime;

   return "<hr><center>Page last modified on $timestamp.</center>";
}

# v0.3 Added by Olivier Chapelle
sub htmlmenu{
  return '
\\HCode{<div id="fixed"><br>}
\\HCode{<a align="right" href="http://www.jmlr.org" target=_top><img align="right" class="jmlr" src="http://jmlr.csail.mit.edu/jmlr.jpg" border="0"></a>}
\\HCode{<p><br><br>}
\\HCode{<p align="right"> <A href="http://www.jmlr.org/"> Home Page </A>}
\\HCode{<p align="right"> <A href="/papers"> Papers </A>}
\\HCode{<p align="right"> <A href="/author-info.html"> Submissions </A>}
\\HCode{<p align="right"> <A href="/news.html"> News </A>}
\\HCode{<p align="right"> <A href="/scope.html"> Scope </A>}
\\HCode{<p align="right"> <A href="/editorial-board.html"> Editorial Board </A>}
\\HCode{<p align="right"> <A href="/announcements.html"> Announcements </A>}
\\HCode{<p align="right"> <A href="/proceedings"> Proceedings </A>}
\\HCode{<p align="right"> <A href="/mloss">Open Source Software</A>}
\\HCode{<p align="right"> <A href="/search-jmlr.html"> Search </A>}
\\HCode{<p align="right"> <A href="/manudb"> Login </A></p>}
\\HCode{<br><br>}
\\HCode{<p align="right"> <A href="http://jmlr.csail.mit.edu/jmlr.xml">}
\\HCode{<img src="http://jmlr.csail.mit.edu/RSS.gif" class="rss" alt="RSS Feed">}
\\HCode{</A>}
\\HCode{</div>}
'
}

# v0.3 new
sub htlatex{
   my ($filename, $cfg) = @_;

   # unicode-related options suggested by Olivier Chapelle

   # v0.31 added latex options in 5th parameter

   my $code = &systemcall(join(' ', 'htlatex',
                  "\"$filename\"",
                  "\"$cfg,uni-html4\"",
                  "\" -cunihtf -utf8\"",
                  '""',
                  "\" $latexopts\""
                 ));

   if ($code)
   {
      die "$appname: htlatex failed with exit code $code.\n";
   }
}

#v0.3 new
sub createjmlrcfg{
   my $cfg = &fname(@_, "jmlr.cfg");

   unless ($execute)
   {
      &messagecall("Skipping creation of '$cfg'\n");
      return;
   }

   open CFG, ">$cfg" or die "$appname: Can't create '$cfg': $!\n";

print CFG <<END_CFG;
\\Preamble{html}
\\begin{document}
\\Css{div.maketitle {text-align:left;}}
\\Css{h2.titleHead {text-align:left;}}
\\Css{. {font-family:verdana,helvetica,sans-serif}}
\\Css{a {text-decoration:none;color:\\#3030a0}}
\\Css{.cmbx-10x-x-109{ font-weight: bold;}}
\\Css{.cmbxti-10x-x-109{ font-weight: bold; font-style: italic;}}
\\Css{\\#fixed {position:absolute; top:0; left:0; width:8em;
height:100\\%;}}
\\Css{\\#content {margin-top:1em; margin-left:10em;
margin-right:0.5em;}}
\\Css{img.jmlr {width: 7em;}}
\\Css{img.rss {width: 2em;}}
\\EndPreamble
END_CFG

# v0.3 Last four \Css lines above added by Olivier Chapelle
   close CFG;
}

#v0.3 new
# copy html from html-src/$dir/ to html/ and rename css file
sub copyhtml{
   my ($dir, $name) = @_;

   my $infile = &fname("html-src", $dir, "$name.html");

   my $outfile = &fname("html", "$name.html");

   unless ($execute)
   {
      &messagecall("Copy '$infile' to '$outfile'\n");
      return;
   }

   open INFD, $infile or die "Can't open '$infile': $!\n";

   open OUTFD, ">$outfile" or die "Can't open '$outfile': $!\n";

   while (<INFD>)
   {
      s/href="$name\.css"/href="jmlr.css"/;

      print OUTFD;
   }

   close OUTFD;

   close INFD;

   # Copy css file

   &copyordie("html-src/$dir/$name.css", "html/jmlr.css");
}

sub parsemainaux{
   my $mainaux = shift;

   &message("Reading '$mainaux'...\n");

   unless (open AUX, "$mainaux")
   {
      if ($execute)
      {
         die "$appname: Can't open '$mainaux' $!\n";
      }
      else
      {
         warn "(Can't open '$mainaux' - skipping)\n";
         return;
      }
   }

   while (<AUX>)
   {
      if (/\\bibdata\b/)
      {
         $main_bibdata = 1;
      }
      elsif (/\\\@jmlr\@import\{(.*)\}\{(.*)\}\{(.*)\}/)
      {
         my $import = 
           {
             label => $1,
             path  => $2,
             name  => $3
           };

         $import->{'name'} =~s/\.(tex|ltx)\Z//;

         push @imports, $import;
      }
      elsif (/\\contentsline\s*\{chapterauthor\}\{(.*)\}\{\}\{\}}\s*$/
        and $#imports > -1)
      {
         $imports[$#imports]->{'author'} = $1;
      }
      elsif (/^\\newlabel\s*\{([^\}]*)jmlrstart\}\{\{([^\}]*)\}\{([^\}]*)\}/)
      {
         my $label = $1;
      
         $pagerefs{$label}->{'start'} = $3;
      }
      elsif (/^\\newlabel\s*\{([^\}]*)jmlrend\}\{\{([^\}]*)\}\{([^\}]*)\}/)
      {
         my $label = $1;

         $pagerefs{$label}->{'end'} = $3;
      }
      elsif ($extractpreface) # v0.3 new
      {
         if (/^\\\@prefacestart\{([^\}]*)\}\{(\d*)\}/)
         {
            $preface_data->{'Start'} = $1;
            $preface_data->{'StartArabic'} = $2;
         }
         elsif (/^\\\@prefaceend\{([^\}]*)\}/)
         {
            $preface_data->{'End'} = $1;
         }
         elsif (/^\\\@prefacefile\{([^\}]*)\}\{([^\}]*)\}/)
         {
            $preface_data->{'File'}    = $1;
            $preface_data->{'OutFile'} = $2;
         }
         elsif (/^\\\@prefaceeditor\{(.*)\}/)
         {
            my $name = $1;
            $name=~s/\\\\.*//;
            push @preface_editors, $name;
         }
      }
   }

   # if preface is to be extracted, has the require data been found?

   if ($extractpreface)
   {
      unless ($preface_data->{'File'})
      {
         warn "$appname: Can't find preface information in aux file.\n",
              "Have you used the preface environment?\n";

         $extractpreface = 0;
      }
   }

   close AUX;
}

sub createprefacefile{
   my ($prefdir, $prefbase) = @_;

   my $prefout = "$prefbase.tex";

   &messagecall("Create preface file '$prefout'\n");

   return unless ($execute);

   # Open preface output file

   open PREFOUT, ">$prefout"
      or die "$appname: Can't open '$prefout': $!\n";

   print PREFOUT "\\batchmode", $eol if ($batchtex or $quiet);
   print PREFOUT "\\makeatletter", $eol;
   print PREFOUT "\\def\\input\@path{{../../}}", $eol;
   print PREFOUT "\\makeatother", $eol;

   # Get the book's preamble

   my $filename = "$main_name$main_suffix";

   open BOOK, $filename
     or die "$appname: Can't open '$filename': $!\n";

   while (<BOOK>)
   {
      if (/\\documentclass/)
      {
         unless (s/^([^%]*)\\documentclass\s*\[(.*)\]/$1\\documentclass[$2,html]/m)
         {
           s/^([^%]*)\\documentclass\s*/$1\\documentclass[html]/m;
         }

         print PREFOUT;
      }
      elsif (/^\\begin{document}/)
      {
         if ($preface_data->{'Start'}=~/^[clxvi]+$/)
         {
            print PREFOUT "\\pagenumbering{roman}%", $eol;
         }
         elsif ($preface_data->{'Start'}=~/^[CLXVI]+$/)
         {
            print PREFOUT "\\pagenumbering{Roman}%", $eol;
         }

         print PREFOUT 
           "\\setcounter{page}{",
           $preface_data->{'StartArabic'},
           "}%", $eol;

         # \hypersetup{draft} is used to suppress links.
         # (Only a partial document so internal links may be
         # dead. Also prevents unwanted tag before the DOCTYPE
         # line in the HTML file.)

         print PREFOUT
               "\\hypersetup{draft}", $eol,
               '\\makeatletter',
               "\\\@openrightfalse\\input{../../$main_name.aux}",
               '\\makeatother', $eol;

         print PREFOUT
               "\\providecommand{\\HCode}[1]{}", $eol,
               "\\title{\\prefacename}", $eol,
               "\\begin{document}", $eol,
               "\\HCode{<div id=\"content\">}", $eol;

         last;
      }
      else
      {
         print PREFOUT;
      }
   }

   close BOOK;

   # Preface file name will have '/' as directory divider

   my $preffile = $preface_data->{'File'};

   if ($dd eq "\\")
   {
      $preffile=~s/\//\\/g;
   }

   open PREFIN, $preffile
     or die "$appname: Can't open '$preffile': $!\n";

   my $scanning  = 0;

   while (<PREFIN>)
   {
      # This is fairly primitive and works best when the begin
      # and end of the environment are on their own line.

      if (/\\begin\{preface\}/)
      {
         print PREFOUT;
         $scanning = 1;
      }
      elsif ($scanning)
      {
         print PREFOUT;

         last if /\\end\{preface\}/;
      }
   }

   close PREFIN;

   print PREFOUT
     "\\HCode{", &htmltimestamp, "}", $eol,
     "\\HCode{</div>}", $eol,
     &htmlmenu,
     "\\end{document}", $eol;

   close PREFOUT;

}

1;


==> sections/01-into.tex <==
\section{Introduction}
\label{sec:intro}

Conformal prediction \citep{shafer2008tutorial,vovk2005algorithmic} is a 
framework that produces predictions with accuracy guarantees.
For a given value of significance level $\epsilon \in (0, 1)$, a conformal predictor is guaranteed to make exactly $\epsilon$ errors in the long run.
This is achieved at a price of a reduction in prediction precision. 
Instead of predicting a single class label, in the case of classification, or a single
number, in the case of regression, a conformal predictor outputs a range prediction, 
that is a set of class labels or an
interval that contains the true value with probability $1 - \epsilon$.
Construction of a conformal predictor with $\epsilon = 0$ is a trivial task.
It is enough to output all class labels or an unbounded interval in case of classification and
regression respectively.
However, such a predictor is of low value, that is, it is not \textit{efficient}.
The question thus is how to guarantee the 
given level of error rate ($\epsilon$) by producing the smallest prediction regions.
This property is achieved via the definition of a proper nonconformity function that 
succeeds to measure the \textit{strangeness} or \textit{nonconformity} of every data
instance \citep{shafer2008tutorial}.

In the case of classification, the \textit{efficiency} of a conformal predictor is often measured in terms of 2 metrics: $avgC$, which stands for the average 
number of predicted class labels per instance, and $oneC$, which stands for 
the fraction of produced singleton predictions. 
Naturally, one would want to minimize $avgC$ and maximize $oneC$ at the
same time.
A recent study by \cite{johansson2017model} showed that \emph{the usage of \textit{margin} as a nonconformity function results in higher $oneC$ and the usage of \textit{inverse probability} (also known as $hinge$) 
%as a nonconformal function 
results in lower
values of $avgC$}\footnote{
In the rest of the text, we will refer to this relationship as a baseline or original pattern
(relationship).
}.
The authors used 21 datasets to demonstrate the statistical significance of this relationship. However, this was done for the case where the baseline classifiers were either  a single artificial neural network (ANN) or an ensemble of bagged ANNs. In this paper, we aim to extend this study with the following contributions:
\begin{enumerate}
    \item We study if the same pattern is present when other
    classification algorithms are used. Our experimental results with 8 
    different classifiers and 9 publicly available datasets show that although
    the previously observed pattern does hold in the majority of the cases, 
    the choice of the best nonconformity function can depend on the analyzed 
    dataset and the chosen underlying classification model. For example, 
    $k$-nearest neighbours classifier performs best with \textit{margin}.
    \textit{Margin} is also the best choice in case of \verb|balance| dataset
    regardless of the chosen classification model.

    \item We propose a method to combine both nonconformity functions. 
    Our experimental evaluation shows that this combination always results 
    in better or the same performance as \textit{inverse probability}, thus 
    allowing to increase the value of $oneC$ and decrease the value of
    $avgC$.
    In some cases, the proposed combination outperforms both 
    \textit{inverse probability} and \textit{margin} in terms of both efficiency metrics.
    
    \item We discuss several aspects of how the accuracy of the baseline 
    classifier can impact the performance of the resulting conformal
    predictor. In particular, if the baseline prediction accuracy is very
    good, then nonconformity
    function has no impact on the efficiency.
    Also, the accuracy of the baseline classifier strongly correlates
    with the fraction of singleton predictions that contain the true label.
    In this way, the accuracy can be an indicator of the usefulness of the $oneC$
    metric.

\end{enumerate}
 
The rest of the paper is organized as follows. In \cref{sec:literature} we discuss related work. \cref{sec:our-approach} is dedicated to the description of the proposed strategy to combine advantages of \textit{margin} and \textit{inverse probability} nonconformity functions. \cref{sec:setup} and \cref{sec:experiments} present the experimental setup and results. Finally, we summarize our work in \cref{sec:conclusions}.






==> sections/02-literature.tex <==
\section{Related work}
\label{sec:literature}

Conformal prediction is a relatively new paradigm developed at the beginning of
2000, see \cite{linusson2021nonconformity} for an overview. It was originally developed for 
transductive setting \citep{vovk2013transductive}. The latter is efficient in terms of 
data usage but is also computationally expensive. Recent studies, including
the current one, focus on \textit{Inductive Conformal Prediction} 
(\textit{ICP})~\citep{papadopoulos2008inductive}. \textit{ICP} trains the 
learning model only once, however a part of the training dataset should be put
aside for model calibration using a predefined nonconformity function.

There are two groups of nonconformity functions: \textit{model-agnostic} and 
\textit{model-dependent}. Model-dependent nonconformity functions are defined
based on the underlying prediction model. Such functions can depend on the
distance to the separating hyperplane in SVM~\citep{balasubramanian2009support}, 
or the distance between instances in KNN classifier~\citep{proedrou2002transductive}.
These nonconformity functions are model-specific, thereby, one can not draw 
generalized conclusions about their behaviour. In a recent study by 
\cite{johansson2017model} it was shown that model-agnostic nonconformity 
functions do have some general characteristics. \textit{Inverse probability} 
nonconformity function, also known as \textit{hinge}, is defined by the
equation $\Delta \left[ h (\vec{x_i}), y_i \right] = 1 - \hat{P}_h(y_i | \vec{x_i})$, where 
$\vec{x_i}$ is the analyzed data instance, $y_i$ is a tentative class label, and
$\hat{P}_h(y_i | \vec{x_i})$ is the probability assigned to this label given the 
instance $\vec{x_i}$ by the underlying classifier $h$. It was shown that 
conformal classifiers based on this metric tend to generate prediction regions
of lower average length ($avgC$). At the same time, \textit{margin} 
nonconformity function results in a larger fraction of singleton predictions
($oneC$). The latter is defined by the following formula 
$\Delta \left[ h (\vec{x_i}), y_i\right] = \max_{y \neq y_i}\hat{P}_h(y | \vec{x_i}) - \hat{P}_h(y_i | \vec{x_i})$,
and it measures how different is the probability of the label $y_i$ from the probability of
another most probable class label. The experimental evaluations in \cite{johansson2017model}, 
however, were performed for a limited number of underlying classification models:
ANN and ensemble of bagged ANNs. To the best of our knowledge, there are no
research works dedicated to the validity analysis of the discovered pattern in the case
of other classification algorithms. %To our opinion, t
This piece of research is
missing to draw global conclusions about the characteristics of these 
nonconformity functions.

Combining characteristics of both \textit{margin} and \textit{inverse
probability} nonconformity functions is a tempting idea. 
In recent years many authors dedicated
their efforts to understand how one can generate more efficient conformal
predictions through a combination of several conformal predictors.
\cite{yang2021finite} and \cite{toccaceli2019combination} studied how to aggregate
conformal 
predictions based on different training algorithms. Various strategies were 
proposed for such combination: via $p$-values~\citep{toccaceli2017combination},
a combination of monotonic conformity scores~\citep{gauraha2018synergy},
majority voting~\citep{cherubin2019majority},  
out-of-bag calibration~\citep{linusson2020efficient}, or via 
established results in classical statistical hypothesis
testing~\citep{toccaceli2019conformal}.
The challenge of every combination of conformal predictors is to retain \textit{validity}, that is 
to achieve the empirical error rate not exceeding the predefined value $\epsilon$.
This property is usually demonstrated experimentally and some authors provide 
guidelines on which values of significance levels should be used for individual
conformal algorithms to achieve the desired validity of the resulting combination.
As opposed to these general approaches, in \cref{sec:our-approach} we
propose a procedure that is based on the 
properties of \textit{margin} and \textit{inverse probability}. Through experiments, we show that this approach
allows combining their characteristics, higher $oneC$ and
lower $avgC$, and retains the validity at the same time.




==> sections/03-our-approach.tex <==
\section{Combination of \textit{inverse probability} and \textit{margin} nonconformity functions}
\label{sec:our-approach}

As was shown by \cite{johansson2017model}, the usage of \textit{inverse probability}
nonconformity function results in less number of predicted class labels on average 
(lower $avgC$), and \textit{margin} results in a  larger fraction of singleton 
predictions (higher $oneC$). In this section, we propose an approach to combine
these properties of the two nonconformity functions. The validity of this method
is studied empirically in \cref{sec:experiments:validity} and its efficiency is 
demonstrated in \cref{sec:experiments:efficiency}.

It is desirable to have more singleton predictions. However, if a singleton prediction
does not contain the true label, then the metric $oneC$ not only loses its
value but also becomes misleading. In \cref{sec:experiments:eff-oneC} we
demonstrate that for some datasets only a half of singleton predictions contain 
the true label. Hence, in our proposed method we decide to take the 
results produced by \textit{inverse probability} nonconformity function as 
a baseline, and then extend them with some singleton predictions resulting 
from the usage of \textit{margin}. 

The proposed procedure is the following.
\textbf{First}, we construct conformal predictors using both nonconformity 
functions separately\footnote{
See \cite{vovk2005algorithmic,shafer2008tutorial,johansson2017model} for
explanation of how conformal predictors are constructed.
}. For the conformal predictor based on \textit{inverse 
probability}, we use the value of $\epsilon$ specified by the user as the
significance level. 
For the conformal predictor based on \textit{margin},
we set the significance level equal to $\epsilon / 2$. This is done to compensate for possible erroneous singleton
predictions produced by \textit{margin} nonconformity function and to achieve the
required level or empirical error rate. \textbf{Second}, for every instance in
the testing or production dataset, we analyze the predictions generated by both 
conformal classifiers. If the conformal classifier based on \textit{margin} outputs 
a singleton and the other conformal classifier does not, then the prediction is
taken from the first model. Otherwise, the output of the conformal classifier 
based on \textit{inverse probability} is used.
Such a combination will perform in the worst case the same as the conformal
predictor based on \textit{inverse probability}. Otherwise, the values of
$oneC$ and/or $avgC$ will be improved, as some non-singleton predictions will
be replaced with singletons. Thereby, in case the validity is preserved, this
combination can be considered as an improved version of the 
\textit{inverse probability} nonconformity function.

In the rest of the paper, we use \textit{M} and \textit{IP} to refer to 
%the conformal classifiers based on 
\textit{margin} and \textit{inverse probability}
respectively. \textit{IP\_M} is used to refer to the combination explained
above.
%referred to as a nonconformity function, although technically it is not.
For simplicity, sometimes \textit{IP\_M} is
referred to as a nonconformity function, although technically it is not.



==> sections/04-1-experimental-setup-dataset.tex <==
\section{Experimental setup}
\label{sec:setup}

%\textcolor{red}{Give names (formulas) to all rows in \cref{tab:datasets-and-results} to reference them in the text.}

To perform experimental analysis, we used the implementation of conformal
prediction framework available from
\textit{nonconformist}\footnote{\url{https://github.com/donlnz/nonconformist}} Python library. 
We followed the general experimental setup from the original paper by \citet{johansson2017model}.
That is we used 10x10-fold cross-validation with 90\% of the data used for 
training and validation of the model, and 10\% used for testing.
The training dataset was further split into a proper training set and a 
calibration set in proportion 4:1.
%, i.e., 80\% of the training set was used for
%actual training of the classification model, and the rest 20\% were used 
%for calibration.
All the results reported below are averaged over the 10x10 folds.
In the original study, the authors used
21 publicly available multi-class datasets from UCI repository~\cite{Dua:2019}.
In this paper, we present not aggregated, but detailed results for every analyzed
dataset.
Such a setup allows us to identify dataset-specific relationships.
%For example, we discovered that for \verb|balance| dataset \textit{margin} is the best choice of nonconformity function. 
That is why we chose 9 representative datasets with different
characteristics from the original list of 21 ones. 
The general information about these datasets, such as the number of instances, attributes, and defined classes is given in the first section of \cref{tab:datasets-and-results}.

\input{paper/sample-papers/sections/04-3-main-results-tab}

The original study by \citet{johansson2017model} analyzed the performance of 
conformal classifiers based on the ANN classification model.
In this paper, we aim to further extend this analysis and use 8 different
classification algorithms as baseline models: Support Vector Machine (SVM), Decision Tree (DT), $k$-Nearest Neighbours (KNN), AdaBoost (Ada), Gaussian Naive Bayes (GNB), Multilayer Perceptron (MPR), Random Forest (RF) and Quadratic Discriminant Analysis (QDA). We used implementations of these algorithms
available from \textit{scikit-learn} Python library. In \cref{tab:algo-params},
we summarize the input parameters of these algorithms unless the default values 
are used.

\begin{table}[htbp]
 % The first argument is the label.
 % The caption goes in the second argument, and the table contents
 % go in the third argument.
\floatconts
  {tab:algo-params}%
  {\caption{Input parameters of classification algorithms}}%
  {
\begin{tabular}{l|l}
Algorithm & Input parameters                                               \\
\hline
SVM       & probability=True                                               \\
DT        & min\_samples\_split=max(5,  5\% of proper training dataset) \\
KNN       & n\_neighbors=5                                                 \\
MPR       & alpha=1, max\_iter=1000                                        \\
RF        & n\_estimators=10, min\_samples\_split=0                         
\end{tabular}
  }
\end{table}

Different classifiers perform differently on different datasets.
We demonstrate this in the second section of \cref{tab:datasets-and-results}.
To calculate the corresponding values, we used the same 10x10-fold cross-validation but without splitting the training set into a proper training set and a
validation set.
\textit{$b\_err$ range} from the first row of this section demonstrates the range of
errors produced by all 8 classification algorithms in the baseline mode\footnote{
In this text we use the \textit{baseline mode} to refer to the standard (non-conformal) prediction.
}. We can 
notice that some datasets are easier to classify, for example, \verb|iris| dataset for which  the maximum error is 6\%. 
At the same time, other datasets are more difficult, for example, \verb|wineW| for which none of the classifiers can produce error less than 45\%.
The performance of classifiers is not uniformly distributed within the given ranges.
This can be seen from the median of baseline error distribution, see row \textit{$b\_err$ median}.
For example, for the  \verb|cars| dataset different classifiers result in errors ranging from 7\% to 96\%. However, the median value of 13 shows that half of them perform relatively well.

%For our analysis we used 3 nonconformity functions: 1) inverse probability, \textit{IP} (also known as \textit{hinge}) defined by the following formula $\Delta \left[h \left( \vec{x_i}, y_i \right) \right] = 1 - \hat{P}_h\left(y_i | \vec{x_i} \right)$; 2) margin (\textit{M}) defined by equation $\Delta \left[h \left( \vec{x_i}, y_i \right) \right] = \max_{y \neq y_i} \hat{P}_h\left(y | \vec{x_i} \right) - \hat{P}_h\left(y_i | \vec{x_i} \right)$; 3) and the combination of \textit{inverse probability} and \textit{margin} as defined in \cref{sec:our-approach}.

All experimental evaluations were performed for 5 different values of significance
level $\epsilon \in \left\{ 0.01, 0.05, 0.1, 0.15, 0.20 \right\}$. For every 
combination of dataset, baseline classification algorithm and $\epsilon$, we 
calculated the values of $oneC$ and $avgC$ with 2 different nonconformity 
functions (\textit{IP} and \textit{M}) and their combination \textit{IP\_M}.
After that, the results were compared to see if any of the nonconformity 
functions or their combination 
results in a more efficient conformal predictor. 
Due to the space limitations of this paper, we present 
detailed results only for 4 datasets highlighted in bold in \cref{tab:datasets-and-results}. 
However, experimental results for all datasets and the 
code used for the experimentation
are available in the related git repository\footnote{
\url{https://github.com/marharyta-aleksandrova/copa-2021-conformal-learning}
}.

%\citet{johansson2017model}

%\citep{johansson2017model}

==> sections/04-2-experiments.tex <==
\section{Experimental results}
\label{sec:experiments}

\subsection{Validity}
\label{sec:experiments:validity}

We start with the analysis of \textit{validity}, that is first we check if 
the produced conformal predictors indeed achieve the required error rate. 
This property was demonstrated in previous works both for \textit{inverse probability} and \textit{margin}.
It is also theoretically guaranteed for any nonconformity function, but not
for a combination of those, like \textit{IP\_M}.
In \cref{tab:validity} we demonstrate the empirical error rates averaged among all datasets. 
As we can see, all conformal predictors are well-calibrated. 
The validity of conformal predictor based on \textit{IP\_M} can be explained 
by the fact, that we add \textit{margin}-based predictions to the 
\textit{IP}-based model only in case when we are very confident about them. 
Recall that the  significance level is set to $\epsilon / 2$ for this case, see
\cref{sec:our-approach}. 
Thereby, the probability to generate enough invalid predictions to surpass 
the allowed error rate $\epsilon$ is very low.

\begin{table}[htbp]
 % The first argument is the label.
 % The caption goes in the second argument, and the table contents
 % go in the third argument.
\floatconts
  {tab:validity}%
  {\caption{Empirical error rates}}%
  {
%\begin{wraptable}{r}{8cm} 
\begin{tabular}{l|lllll}
\textbf{eps:}   & \textbf{0.01} & \textbf{0.05} & \textbf{0.10} & \textbf{0.15} & \textbf{0.20} \\
\hline
\textit{IP}    & 0.01          & 0.05          & 0.09         & 0.14          & 0.19         \\
\textit{IP\_M} & 0.01          & 0.05          & 0.10         & 0.15          & 0.19         \\
\textit{M}     & 0.01          & 0.05          & 0.10         & 0.15          & 0.19        
\end{tabular}
%\end{wraptable}
  }
\end{table}


%\begin{table}[htbp]
 % The first argument is the label.
 % The caption goes in the second argument, and the table contents
 % go in the third argument.
%\floatconts
%  {tab:validity}%
%  {\caption{Emperical error rates}}%
%  {
%\begin{tabular}{l|llllll}
%\textbf{eps}   & \textbf{0.01} & \textbf{0.03} & \textbf{0.05} & \textbf{0.10} & \textbf{0.15} & \textbf{0.20} \\
%\hline
%\textit{IP}    & 0.01          & 0.03          & 0.05          & 0.09         & 0.14          & 0.19         \\
%\textit{IP\_M} & 0.01          & 0.03          & 0.05          & 0.10         & 0.15          & 0.19         \\
%\textit{M}     & 0.01          & 0.03          & 0.05          & 0.10         & 0.15          & 0.19        
%\end{tabular}
%  }
%\end{table}

\subsection{Informativeness of $oneC$}
\label{sec:experiments:eff-oneC}

In \cref{sec:our-approach}, we discussed the issue that can happen with $oneC$ 
metric. Indeed, if a large portion of predicted singletons does not contain the 
true label, then this metric can be misleading.
We calculated the ratio of the number of singleton predictions that contain 
the true label to the overall number of singleton predictors for different
setups and algorithms. We denote this value as $E\_oneC$ from \textit{effective $oneC$}. The corresponding results are presented in 
section 3 of \cref{tab:datasets-and-results}.

%First, we calculated the ratio of the number of correct singleton predictors to the total number of singleton predictors produced by a conformal classifier. 
The first row of this section shows the averaged value of $E\_oneC$ over all 5
values of $\epsilon$ and 3 nonconformity functions.
We can notice that this value is very different for different datasets ranging
from 0.98 for \verb|iris| to only 0.50 for \verb|wineW|. 
This means that for \verb|wineW| on average half of the produced singleton 
predictions do not contain the true label. In real applications, this
prediction can be more confusing than a prediction with multiple labels.

We can notice that there is a certain correlation between the mean value of 
$E\_oneC$ and the difficulty of the dataset for the baseline classifiers 
($b\_err$). 
To analyze this relationship, we calculated the value of correlation between 
the corresponding characteristics.
The results are presented in the third row \textit{corr. $b\_acc$}.
We can see that for 5 of 9 datasets (56\%) the correlation is above 0.9. 
This holds for \verb|iris|, \verb|user|, \verb|cars|, \verb|wave|, and \verb|yeast| datasets.
For 2 more datasets (\verb|balance| and \verb|wineW|), the correlation coefficient is approximately 0.8.
For \verb|glass| dataset, it is equal to 0.69, and only for \verb|wineR| the correlation is as low as 0.27.
These results show a strong relationship between the baseline error of the underlying classification model and the correctness of singleton predictions.
%It means that for a well performing classifier, we can expect a large
%portion of singleton predictions to be correct.
%However, in case of less well performing baseline classifier, only a half of %the resulting singleton prediction might contain the true label.

Finally, to check if $E\_oneC$ depends on the chosen nonconformity function, we averaged the results separately for different non-conformity functions and then calculated the standard deviation of the resulting three values.
The corresponding results are presented in the second row \textit{mean-std}.
We notice that \textit{mean-std} is very low for all datasets.
This indicates that $E\_oneC$ does not depend on the choice of nonconformity function.

\subsection{Efficiency of different nonconformity functions}
\label{sec:experiments:efficiency}

In this section, we study the relationship between different nonconformity functions and the effectiveness of the resulting conformal predictors. 
For every combination of a dataset, a baseline classifier, and a value of $\epsilon$,
we calculate the values of $oneC$ and $avgC$. For visual analysis, the corresponding results
are plotted using the same format as in \cref{fig:iris,fig:glass}. Such figures contain information about
the distribution of instances between classes (plots \textit{a}), the baseline
error rate of all classification algorithms $b\_err$ (plots \textit{b}), and the 
corresponding values of the efficiency metrics (plots from \textit{c} to \textit{j}).
The latter group of plots contains three lines corresponding to \textit{margin} (dashed line),
\textit{inverse probability} (dash and dot line) and their combination \textit{IP\_M}
(thin solid line).

Further, we evaluate how significant are the differences between different nonconformity 
functions. The corresponding results are summarized in the same format as presented in  \cref{tab:glass}.
Here, for every baseline classifier and value of $\epsilon$, we present a comparison matrix.
A value in the matrix shows if the row setup is better (indicated with $+$) or
worse (indicated with $-$) than the column setup. The star indicates if the 
detected difference is statistically significant\footnote{Statistical significance was 
estimated using Student's t-test with $\alpha = 0.05$.}.
To avoid too small differences, we put a sign into the matrix only if the corresponding
difference is above the threshold of 2\%\footnote{For 100\% we take the value of 1 
for $oneC$ and the total number of classes for $avgC$. These are the maximum values of
these two metrics.} or it is statistically significant.
For example, from \cref{tab:glass} we can see that \textit{margin} results in better values of $oneC$ than
\textit{IP} and \textit{IP\_M} for SVM with $\epsilon=0.05$.
These results are also statistically significant, as indicated by a *.
At the same time, for $\epsilon=0.1$ \textit{margin} improves the results of 
\textit{IP\_M} by at least 2\%.
However, this difference is not statistically significant.
Section 4 of \cref{tab:datasets-and-results} shows the fraction of setups, for which we can observe  a
difference between the performance of conformal classifiers with different nonconformity functions 
either by exceeding the threshold of 2\% (\textit{thres.}) or observing statistical significance (\textit{stat.}). 
These values are calculated as follows. For every dataset, we have 40 setups (5 values of $\epsilon$ x
8 baseline classifiers). Each such setup corresponds to one matrix for $oneC$ and one 
matrix for $avgC$ in significance tables.
%like \cref{tab:glass}. 
We calculate how many of these matrices either have at least one $+$ or $-$, or have at least one
statistically significant result.
After that, the calculated number is divided over 40.
%We provide detailed analysis of the results for those datasets in \cref{tab:datasets-and-results} that are highlighted in bold. 


Using such information %provided 
for all datasets,
%in figures like \cref{fig:glass} and tables like \cref{tab:glass},
we can analyze the efficiency of conformal classifiers for different nonconformity functions
and identify which of them %nonconformity functions
perform better.
The corresponding findings are summarized in section 5 of \cref{tab:datasets-and-results}.
This part of the table shows the deviations from the pattern originally observed by \cite{johansson2017model}.
In our experiments we observed the following 3 deviations:
1) \textbf{\textit{M} is the best}: \textit{margin} can produce both higher values of $oneC$ and lower values of $avgC$, that is \textit{margin} is the best choice of nonconformity function;
2) \textbf{\textit{IP} is the best}: \textit{inverse probability} is the best choice of
nonconformity function;
3) \textbf{\textit{IP\_M} is the best}: the combination of \textit{M} and \textit{IP} produces 
the best results in terms of both efficiency metrics.
Additionally, our experiments show that \textit{IP\_M} never performs worse than \textit{IP} 
(\textit{IP\_M} $>$ \textit{IP}).
Note also, that we never observed the inverse pattern, that is \textit{inverse probability} resulting 
in higher values of $oneC$ and \textit{margin} resulting in lower values of $avgC$ at the same time. 
In the rest of this section, we demonstrate our main findings on the examples of 4 datasets
highlighted in bold in \cref{tab:datasets-and-results}. The general conclusions are discussed
in \cref{sec:experiments:summary}.



%\subsubsection{iris}

%Let us start the analysis for the first dataset - . 
\textbf{IRIS}. The results for \verb|iris| dataset are presented in \cref{fig:iris}. 
As we can see from the plots comparing $oneC$ and $avgC$, there is almost no difference
and all 3 nonconformity functions produce the same results.
This is also reflected in section 4 of \cref{tab:datasets-and-results}.
Only for 5\% of setups we can observe a difference in terms of $oneC$, see performance of RF in \cref{fig:iris:oneC-RF-QDA}.
The difference in $avgC$ is observed even less often, only in 2.5\% of setups, see results for GNP in \cref{fig:iris:avgC-GNB-MPR}. 
Statistically significant differences are never observed.
This means that the table with the significance of results like \cref{tab:glass} for this dataset is
almost empty. That is why we do not present it in the paper.
As expected, not many patterns can be observed in this case. 
The only pattern that we observe, is \textit{IP\_M} $>$ \textit{IP}.
Note, that this dataset is perfectly balanced, see \cref{fig:iris:dist-class} and all classifiers have very good performance with maximum error not exceeding 6\%, see \cref{tab:datasets-and-results} and \cref{fig:iris:baseline-error}.
We can also notice that there is a relationship between the baseline error of the classifier and the 
efficiency of the resulting conformal predictor: better classifiers tend to produce conformal 
predictors of better quality.
The 3 worst baseline predictors DT, Ada, and RF also produce conformal predictors with lower values of $oneC$, see \cref{fig:iris:oneC-SVM-DT,fig:iris:oneC-KNN-Ada,fig:iris:oneC-RF-QDA} and larger values of $avgC$, see \cref{fig:iris:avgC-SVM-DT,fig:iris:avgC-SVM-DT,fig:iris:avgC-RF-QDA}.


\input{paper/sample-papers/sections/4-iris-data/plots}

%\subsubsection{glass}

\textbf{GLASS}.
Next, we analyze the results for \verb|glass| dataset presented in \cref{fig:glass} and 
\cref{tab:glass}. This dataset is unbalanced, see \cref{fig:glass:dist-class} and 
different classifiers have different performance with baseline error ranging from 24\% for RF to 92\%
for QDA, see \cref{fig:glass:baseline-error}. As it was observed for \verb|iris| dataset, those 
classifiers that perform better in the baseline scenario also tend to produce more efficient 
conformal predictors.
For example, see the results for RF in \cref{fig:glass:oneC-RF-QDA,fig:glass:avgC-RF-QDA}, and the 
results for KNN in \cref{fig:glass:oneC-KNN-Ada,fig:glass:avgC-KNN-Ada}.
At the same time, classifiers that perform badly in the baseline scenario produce conformal 
predictors of low quality, see results for QDA in \cref{fig:glass:oneC-RF-QDA,fig:glass:avgC-RF-QDA}.
There are also exceptions, but they are less numerous. 
For example, for this dataset the baseline performance of the DT classifier is good ($b\_err \approx 
30\%$), however, the resulting conformal classifier is less efficient than the one based on SVM with 
$b\_err > 60\%$.
For this dataset, we can also observe a clear difference in performance depending on which 
nonconformity function is used.
This is summarized in \cref{tab:glass}. 
Analyzing the results presented in this table, we can observe the following patterns.
1) For KNN and DT-based conformal predictors \textit{margin} is the best choice of nonconformity function.
Indeed, this is reflected in \cref{fig:glass:oneC-KNN-Ada,fig:glass:oneC-SVM-DT} (\textit{margin} 
results in higher values of $oneC$) and  \cref{fig:glass:avgC-KNN-Ada,fig:glass:avgC-SVM-DT} 
(\textit{margin} also results in lower values of $avgC$).
This pattern is also shown in \cref{tab:glass} in comparison matrices corresponding to KNN and DT algorithms. 
We can see that in all comparison matrices, there is a $+$ in rows corresponding to \textit{margin}
indicating that it outperforms both \textit{IP} and \textit{IP\_M},
except $avgC$ for KNN with $\epsilon=0.2$.
2) For MPR \textit{IP\_M} is the best choice of nonconformity function. 
This is reflected in the corresponding comparison matrices of \cref{tab:glass}, from which we can see
that \textit{IP\_M} results in higher values of $oneC$ and lower values of $avgC$ at the same time.
This is also visible in \cref{fig:glass:oneC-GNB-MPR,fig:glass:avgC-GNB-MPR}.
3) Finally, we never observe \textit{IP\_M} being outperformed by \textit{IP}. In the inverse direction,
however, \textit{IP\_M} does improve the results of \textit{IP}.
For example, for SVM with $\epsilon=0.05$ or $\epsilon=0.1$ \textit{IP\_M} allows to achieve better 
values of $oneC$ and this improvement is also statistically significant.
\input{paper/sample-papers/sections/3-glass-data/plots}
\input{paper/sample-papers/sections/3-glass-data/table_threshold}

\textbf{WAVE.}
The results for \verb|wave| dataset are presented in \cref{fig:wave} and \cref{tab:wave}.
This dataset is balanced, see \cref{fig:wave:baseline-error}, and overall performance of classifies 
is quite good, see \cref{fig:wave:baseline-error}. There is only one classifier, DT, wich results in 
$b\_err > 20\%$. 
As it was also noted for \verb|iris|, when classifiers have good baseline performance, the 
difference between different nonconformity functions diminishes.
This is reflected in the reduction of values in section 4 of \cref{tab:datasets-and-results} (25\%, 
27.5\%, 30\%, and 47.5\%) as compared to the corresponding values for \verb|glass| dataset 
(75\%, 67.5\%, 50\%, and 37.5\%).
We can observe visual differences in \cref{fig:wave} only for DT, Ada, GNB, and RF.
No difference is observed for KNN, however, despite it having a comparable value of $b\_err$. 
For this dataset, we can also see that \textit{margin} results in best performance for $\epsilon \in \{ 0.1, 0.15, 0.2\}$ when Ada classifier is used.
This improvement is also statistically significant, see \cref{tab:wave}. 
In the case of $\epsilon = 0.01$ however, the best performance is achieved by \textit{IP} nonconformity 
function, and this result is also statistically significant.
Further, \textit{IP\_M} is the best choice for RF classifier with statistical significance of the improvement in most of the settings.

\input{paper/sample-papers/sections/6-wave-data/plots}
\input{paper/sample-papers/sections/6-wave-data/table_threshold}



\textbf{BALANCE.}
The case of \verb|balance| dataset is very interesting: %$, 
%because, as we will see,
for most of the 
classification models \textit{margin} is always the best choice of nonconformity function.
As reflected in \cref{tab:balance} and supported by \cref{fig:balance}, these differences
are mostly statistically significant.
The only cases for which the original pattern holds are SVM with all values of $\epsilon$ 
and QDA with $\epsilon=0.05$. For this dataset, we also observe differences between different
nonconformity functions despite the relatively good performance of many classifiers. 
%This was opposite for \textit{wave} dataset. Maybe it is related to the fact that margin is best choice here.

\input{paper/sample-papers/sections/1-balance-data/plots}
\input{paper/sample-papers/sections/1-balance-data/table_threshold}

%\textbf{YEAST.}
%The last dataset that we will consider is \textit{yeast} with results presented in \cref{fig:yeast} and \cref{tab:yeast}.
%This dataset that has the largest number of classes (10) and it is highly unbalanced, see \
%cref{fig:yeast:dist-class}. 
%This is one of the most difficult datasets in the baseline setting with $b\_err$ ranging from 40\% for SVM and MPR to 87\% for QDA, see \cref{fig:yeast:baseline-error}.
%For this dataset, we again observe cases when \textit{margin} outperforms all other nonconformity function: KNN with $\epsilon \in \{ 0.05, 0.1, 0.15 \}$, DT with $\epsilon=0.05$, Ada with $\epsilon \in \{ 0.15, 0.2 \}$ and QDA with $\epsilon \in \{ 0.15, 0.2 \}$.
%For the majority of these cases, the difference is statistically significant, see \cref{tab:yeast}.
%For this dataset, we can also observe that \textit{IP\_M} allows to significantly improve the values
%of $oneC$ as compared to \textit{inverse probability} nonconformity function.
%It also usually improves the value of $avgC$, being the best choice in terms of this unless 
%\textit{margin} provides better results. For example, see results for SVM (\cref{fig:yeast:oneC-SVM-DT,fig:yeast:avgC-SVM-DT}), GNP and MPR (\cref{fig:yeast:oneC-GNB-MPR,fig:yeast:avgC-GNB-MPR}), and RF (\cref{fig:yeast:oneC-RF-QDA,fig:yeast:avgC-RF-QDA}).  

%\input{paper/sample-papers/sections/9-yeast-data/plots}
%\input{paper/sample-papers/sections/9-yeast-data/table_threshold}

\subsection{Summary of results}
\label{sec:experiments:summary}

In this subsection we summarize the findings from our experimental results shown in \cref{tab:datasets-and-results}.

    %\textbf{\textit{Margin} can be the best non-conformity function}. 
    As we saw, \textbf{\textit{margin} can be the best choice of nonconformity function} for some datasets (\verb|balance| dataset) or some algorithms. 
    An interesting fact is that for almost all datasets KNN-based conformal predictor works best with \textit{margin} in terms of both $oneC$ and $avgC$.
    %For \textit{yeast} dataset this is also observed for 3 of 4 values of $\epsilon$ which results in different values of efficiency metrics, see \cref{tab:yeast}. 
    This pattern was not observed only for \verb|iris| and \verb|wave| datasets as all 
    nonconfomity functions result in the same values of $oneC$ and $avgC$ in case KNN is used. This observation
    suggests that some classification algorithms and datasets might \textit{prefer} particular
    nonconformity functions.
    
     \textbf{\textit{Inverse probability} is almost never the best nonconformity function}.
    We observed that \textit{margin} can result in the best conformal classifiers in terms of both efficiency metrics. 
    However, it almost never happens with \textit{inverse probability} function.
    In our experiments, this was observed only for Ada classifier for \verb|user| dataset with $\epsilon = 0.15$ and \verb|wave| dataset with $\epsilon = 0.01$.
    
     \textbf{\textit{IP\_M} improves \textit{IP}}. In none of our experiments, we  observed \textit{IP\_M} being outperformed by \textit{IP}.
    \textit{IP\_M} improves $oneC$ and $avgC$ as compared to \textit{IP} or produces the same values of these metrics.
    This is expected, as \textit{IP\_M} is basically an \textit{IP} measure with some non-singleton predictions replaced with singletons.
    This replacement naturally increases $oneC$ and decreases $avgC$.
    The fact that \textit{IP\_M} also results in valid predictions respecting the imposed value of maximum error rate $\epsilon$, as was demonstrated in \cref{tab:validity}, proves the utility of this approach.
    Additionally, in some cases \textit{IP\_M} produces better results than both \textit{margin} and \textit{inverse probability} in terms of both efficiency metrics.
    This was observed for \verb|glass| dataset with MPR, and for \verb|cars| and \verb|wave| datasets with RF.
    
    \textbf{The baseline pattern holds for the majority of the cases}. 
    In our experimental results, we discussed only the cases which deviate from the baseline pattern.
    As we saw, such cases do exist, and a
    particular nonconformity function produces the best values of both metrics for some baseline classifiers or some datasets. 
    However, in most of the cases when the difference between nonconformity functions is observed,
    \textit{margin} results in better values of $oneC$ and \textit{inverse probability} results in 
    better values of $avgC$.
    Also, we never observed an inverse pattern, that is \textit{inverse probability} resulting in 
    higher values of $oneC$ and \textit{margin} resulting in lower values of $avgC$ at the same 
    time.
    This supports the main finding of the original paper by \citet{johansson2017model}.
    
    \textbf{$oneC$ is not always useful.}
    As was discussed in \cref{sec:experiments:eff-oneC}, metric $oneC$ can be misleading.
    For some of the datasets, only half of the singleton predictions contain the true label.
    In such cases, the minimization of $avgC$ is preferred over the maximization of $oneC$.
    We also showed that the fraction of correct singleton predictions strongly correlates with the 
    performance of the chosen classifier in the baseline scenario.
    It means that by analyzing this performance, we can estimate how accurate the singleton 
    predictors will be and we can decide which efficiency metric should be considered more important.
    Also, it was shown that the choice of nonconformity function has little impact on 
    the fraction of correct singleton predictions $E\_oneC$.
    
    \textbf{The baseline performance of the chosen classifier impacts the efficiency of the conformal predictor}.
        In our experiments, we observed that if the performance of the baseline classifier is good, then the choice of nonconformity function tends to have no impact on the efficiency of the resulting conformal classifier. This is the case for \verb|iris| and \verb|wave| datasets.
        In the case of \verb|balance| dataset, this relationship is less prominent and \textit{margin} always outperforms \textit{IP} and \textit{IP\_M}.
        This can be related to the fact that this dataset is unbalanced as opposed to the two other datasets.
        In this case, the classifier can have problems generating predictions for the minority classes. This will not be reflected in the baseline error due to the little number of instances in these classes.
        The baseline performance of the underlying classification model also has a direct impact on the efficiency of the resulting conformal classifier. 
        Except for some cases, soon after the value of $\epsilon$ reaches the value of $b\_err$,
        metric $oneC$ reaches its maximum and starts decreasing.
        At the same time, the value of $avgC$ reaches 1 and further decreases,
        see, for example, results for \verb|iris| dataset presented in \cref{fig:iris}.
        This observation makes sense.
        When $\epsilon > b\_err$, the conformal classifier is allowed to make more mistakes than it does in the baseline scenario. 
        This can be only achieved by generating empty predictions.
        For such values of $\epsilon$, more and more predictions will be singletons or empty what results in the decrease of $oneC$ and $avgC$ below 1.





%\input{sections/04-04-iris}
%\input{sections/04-05-user}


%\input{sections/04-03-glass}
%\input{sections/04-02-cars}
%\input{sections/04-06-wave}


%\input{sections/04-01-balance}
%\input{sections/04-07-wineR}
%\input{sections/04-08-wineW}
%\input{sections/04-09-yeast}





==> sections/04-3-main-results-tab.tex <==
\begin{sidewaystable}[htbp]
%\scriptsize
\floatconts
  {tab:datasets-and-results}
  {\caption{Characteristics of the datasets and summarization of results}}
  {
\begin{tabular}{l|l|l|l|l|l|l|l|l|l|l|l}
                            \multicolumn{2}{l|}{\scriptsize{Section}} & \multicolumn{1}{r|}{\textbf{Datasets} }                                & \textbf{iris} & \textit{user} & \textbf{glass} & \textit{cars} & \textbf{wave} & \textbf{balance} & \textit{wineR} & \textit{wineW} & \textit{yeast}            \\
\hline
\hline
\hline
\multirow{4}{*}{1} & \multirow{4}{*}{\rotatebox[origin=c]{90}{info}} & \# instances                    & 150           & 403           & 214            & 1728          & 5000          & 625              & 1599           & 4898           & 1484                      \\
                            & & \# attributes                   & 4             & 5             & 9              & 6             & 21            & 4                & 11             & 11             & 8                         \\
                            & & \# classes                      & 3             & 4             & 6              & 4             & 3             & 3                & 6              & 7              & 10                        \\
                            & & balanced                        & Y             & mostly        & N              & N             & Y             & N                & N              & N              & N                         \\
\hline
\hline
\hline
\multirow{2}{*}{2} & \multicolumn{2}{l|}{$b\_err$ range, \%}                           & 2-6           & 5-32          & 24-92          & 7-96          & 13-25         & 3-21             & 38-50          & 45-58          & 40-87                     \\
& \multicolumn{2}{l|}{$b\_err$ median, \%}                          & 4             & 7             & 48             & 13            & 17            & 10               & 45             & 53             & 44                        \\
\hline
\hline
\hline
\multirow{3}{*}{3} & \multirow{3}{*}{\rotatebox[origin=c]{90}{ $E\_oneC$}} & mean                      & 0.98          & 0.93          & 0.63           & 0.88          & 0.90          & 0.96             & 0.52           & 0.50           & 0.56                      \\
                            & & mean-std                        & 0.00          & 0.00          & 0.02           & 0.00          & 0.00          & 0.00             & 0.03           & 0.02           & 0.02                      \\
                            & & corr. $b\_acc$               & 0.92          & 0.98          & 0.69           & 0.93          & 0.92          & 0.80             & 0.27           & 0.78           & 0.97                      \\
\hline
\hline
\hline
\multirow{4}{*}{4}& \multirow{2}{*}{\rotatebox[origin=c]{90}{thres.}}      & $oneC$,\%                       & 5             & 15            & 75             & 47.5          & 25            & 67.5             & 72.5           & 65             & 77.5                      \\
                            & & $avgC$,\%                       & 2.5           & 22.5          & 67.5           & 37.5          & 27.5          & 42.5             & 80             & 77.5           & 82.5                      \\\cline{2-12}
%\hline
&\multirow{2}{*}{\rotatebox[origin=c]{90}{stat.}}       & $oneC$,\%                       &               & 5             & 50             & 45            & 30            & 55               & 82.5           & 85             & 85                        \\
                            & & $avgC$,\%                       &               & 17.5          & 37.5           & 45            & 47.5          & 50               & 82.5           & 77.5           & 77.5                      \\
\hline
\hline
\hline
\multirow{6}{*}{5} &\multirow{6}{*}{\rotatebox[origin=c]{90}{patterns}}    & \multirow{3}{*}{\textit{M} is the best} &               & {\scriptsize \textbf{KNN}}           & {\scriptsize \textbf{\textbf{KNN}},}        & {\scriptsize \textbf{\textbf{KNN}}}           & {\scriptsize Ada}         & {\scriptsize \textbf{\textbf{KNN}}, DT, RF,}    & {\scriptsize \textbf{\textbf{KNN}}}            & { \scriptsize \textbf{\textbf{KNN}}}            & {\scriptsize \textbf{\textbf{KNN}}(0.05, 0.1, 0.15),}     \\
                             &&                                 &               &               & {\scriptsize DT}               &               & {\scriptsize (0.1, 
                             0.15,}      & {\scriptsize GNP, MPR,}        & \scriptsize{(0.05, 0.1),}    & {\scriptsize (0.05, 0.1)}     & {\scriptsize DT(0.05), Ada(0.15,} \\
                             &&                                 &               &               &                &               & {\scriptsize 0.20)}   & {\scriptsize Ada, QDA }         & {\scriptsize DT(0.05) }      &                & {\scriptsize  0.2), QDA(0.15, 0.2)}            \\\cline{3-12}
                             && \textit{IP} is the best                      &               & {\scriptsize Ada(0.15)}     &                &               & {\scriptsize Ada(0.01)}     &                  &                &                &                           \\\cline{3-12}
                             && \textit{IP\_M} is the best                   &               &               & {\scriptsize MPR}            & {\scriptsize RF}           & {\scriptsize RF }          &                  &                &                &                           \\\cline{3-12}
                             && \textit{IP\_M} $>$ \textit{IP}               & Y             & Y             & Y              & Y             & Y             & Y                & Y              & Y              & Y\\    
\hline
\hline
\hline
%6 & \multicolumn{2}{l|}{credibility \& $b\_err$}                       & Y              & Y          %   &                & Y             & Y             & Y                &                &            %    &                           \\
%\hline
%\hline
%\hline
%                             7 & \multicolumn{2}{c|}{$b\_acc \uparrow \Rightarrow $ eff. $\uparrow$}                & ?             & ?             & ?              & ?             & ?             & ?                & ?              & ?              & ?\\
\end{tabular}
  }
\end{sidewaystable}


==> sections/05-conclusions.tex <==
\section{Conclusions and Future Work}
\label{sec:conclusions}

The objective of this paper is to further extend the recent results presented by
\cite{johansson2017model} stating that there is a relationship between different model-agnostic
nonconformity functions and the values of $oneC$ and $avgC$. Through an empirical evaluation with 
ANN-based conformal predictors, 
the authors showed that the usage of \textit{margin} nonconformity function results in higher values of
$oneC$ and \textit{inverse probability} nonconformity function allows to achieve lower values
of $avgC$. Next, it is up to the user to decide which metric should be preferred and to choose an
appropriate nonconformity function.
We aim to check if the same pattern would be observed for other classification algorithms.
Through experimental evaluation we showed that the previously observed pattern is supported in most of
the cases, however, some classifiers and/or datasets clearly `prefer' \textit{margin}.
This was observed for KNN classifier and \verb|balance| dataset.
At the same time, \textit{inverse probability} is the best choice of nonconformity function only in
a very small number of cases. This can be considered an exception rather than a rule.

We also proposed a method to combine \textit{margin} and \textit{inverse probability} into a model 
that we denote by \textit{IP\_M}. We showed that \textit{IP\_M} can be considered as an improved 
version of conformal predictor based on \textit{IP} making this approach preferable for minimization
of $avgC$ in most of the cases. Additionally, it was shown that \textit{IP\_M} can be the best
model in terms of both $oneC$ and $avgC$ in some cases: MPR-based conformal predictors
for \verb|glass| dataset, and RF-based conformal predictors for \verb|cars| and \verb|wave|.
The validity of this approach was confirmed experimentally.

Finally, we studied how the effectiveness of the baseline classification algorithm on the given
dataset can impact the efficiency of the related conformal predictor. In particular, we showed
that a fraction of singleton predictions that contain the true label correlates strongly with 
the baseline accuracy. This observation suggests that $oneC$ metric can be misleading in
the case of a poorly performing baseline classifier. Our experiments also demonstrate that usually
classification algorithms with higher values of baseline accuracy result in more efficient
conformal predictors.

Some directions for future work are the following. It can be interesting to confirm that KNN-based
conformal predictors work better with \textit{margin} nonconformity function in the case of other 
datasets. Further, we would like to study which characteristics of baseline classifiers and
datasets make them work better with a particular nonconformity function. For example, for
\verb|balance| dataset SVM-based conformal predictor is the only one that does not `prefer'
\textit{margin} and follows the originally observed pattern. Next, we would like to investigate 
if the proposed method for combining \textit{margin} and \textit{inverse probability} can be improved
using the latest results in assembling conformal predictors such as in \cite{toccaceli2019conformal}. 


%\begin{itemize}
    
%    \item - In this article a very generic method is proposed which takes advantage of a well-established result in Classical Statistical Hypothesis Testing, the NeymanPearson Lemma
    
%    \item \cite{vovk2014criteria} - This paper investigates properties of various criteria of efficiency of conformal prediction in the case of classification.
    
%    \item how to identify the best combination ($\epsilon$ for margin)
%\end{itemize}

==> sections/1-balance-data/plots.tex <==
\begin{figure}[htbp]
\floatconts
  {fig:balance}
  {\caption{Results for \textit{balance}: \textit{M} - dashed line,
  \textit{IP} - dash and dot line, \textit{IP\_M} - thin line}}
  {%
    \subfigure[Distribution between classes]{
    \label{fig:balance:dist-class}%
    \includeteximage{plots/balance-dist-class}
    }%
    \qquad
    \subfigure[Baseline error]{\label{fig:square}%
      \includeteximage{plots/balance-baseline-error}
      }
    \qquad
    \subfigure[$oneC$: SVM and DT]{\label{fig:square}%
      \includeteximage{plots/balance-oneC-0}
      %\includeteximage{plots/balance-dist-class}
      }
    \qquad
    \subfigure[$avgC$: SVM and DT]{\label{fig:square}%
      \includeteximage{plots/balance-avgC-0}
      }
    \qquad
    \subfigure[$oneC$: KNN and Ada]{\label{fig:square}%
      \includeteximage{plots/balance-oneC-2}
      }
    \qquad
    \subfigure[$avgC$: KNN and Ada]{\label{fig:square}%
      \includeteximage{plots/balance-avgC-2}
      }
    \qquad
    \subfigure[$oneC$: GNB and MPR]{\label{fig:square}%
      \includeteximage{plots/balance-oneC-4}
      }
    \qquad
    \subfigure[$avgC$: GNB and MPR]{\label{fig:square}%
      \includeteximage{plots/balance-avgC-4}
      }
    \qquad
    \subfigure[$oneC$: RF and QDA]{\label{fig:square}%
      \includeteximage{plots/balance-oneC-6}
      }
    \qquad
    \subfigure[$avgC$: RF and QDA]{\label{fig:square}%
      \includeteximage{plots/balance-avgC-6}
      }
  }
\end{figure}

==> sections/1-balance-data/table_threshold.tex <==
\begin{table}[htbp]
\scriptsize
 % The first argument is the label.
 % The caption goes in the second argument, and the table contents
 % go in the third argument.
\floatconts
  {tab:balance}%
  {\caption{Significance of results for the \textit{balance} dataset}}%
  {
\begin{tabular}{cl|lll|lll|lll|lll|lll}
             && \multicolumn{3}{c|}{$\epsilon=0.01$} & \multicolumn{3}{c|}{$\epsilon=0.05$} & \multicolumn{3}{c|}{$\epsilon=0.1$} & \multicolumn{3}{c|}{$\epsilon=0.15$} & \multicolumn{3}{c}{$\epsilon=0.2$} \\
\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            & $-$*       &            &            & $-$*       &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            & $-$*       &            &            & $-$*       &            &            &            &            &            &            &            &            &             \\
&m            & $+$*       & $+$*       &            & $+$*       & $+$*       &            &            &            &            &            &            &            &            &            &             \\

\hline
\multicolumn{2}{l|}{\textbf{SVM}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            & $+$*       &            &            &            &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            & $+$*       &            &            &            &            &            &            &            &            &            &            &            &             \\
&m            & $-$*       & $-$*       &            &            &            &            &            &            &            &            &            &            &            &            &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            & $-$        &            & $-$        & $-$*       &            &            & $-$*       &            &            & $-$*       &            &            & $-$*        \\
&ip\_m        &            &            & $-$        & $+$        &            & $-$*       &            &            & $-$*       &            &            & $-$*       &            &            & $-$         \\
&m            & $+$        & $+$        &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$        &             \\

\hline
\multicolumn{2}{l|}{\textbf{DT}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            &            &            & $-$        & $-$*       &            &            & $-$*       &            &            &            &            &            &             \\
&ip\_m        &            &            &            & $+$        &            & $-$*       &            &            & $-$*       &            &            &            &            &            &             \\
&m            &            &            &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            &            &            &            &            &            &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            & $-$*       &            & $-$*       & $-$*       &            &            & $-$*       &            &            & $-$*       &            &            & $-$*        \\
&ip\_m        &            &            & $-$*       & $+$*       &            & $-$*       &            &            & $-$*       &            &            & $-$*       &            &            & $-$*        \\
&m            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &             \\

\hline
\multicolumn{2}{l|}{\textbf{KNN}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            & $-$*       &            & $-$*       & $-$*       &            &            & $-$*       &            &            & $-$*       &            &            & $-$*        \\
&ip\_m        &            &            & $-$*       & $+$*       &            & $-$*       &            &            & $-$*       &            &            & $-$*       &            &            & $-$*        \\
&m            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*        \\
&ip\_m        &            &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            &             \\
&m            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       &            &             \\

\hline
\multicolumn{2}{l|}{\textbf{Ada}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*        \\
&ip\_m        &            &            & $-$*       & $+$*       &            &            & $+$*       &            &            & $+$*       &            &            & $+$*       &            &             \\
&m            & $+$*       & $+$*       &            & $+$*       &            &            & $+$*       &            &            & $+$*       &            &            & $+$*       &            &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            & $-$*       &            & $-$*       & $-$*       &            &            & $-$        &            &            &            &            &            &             \\
&ip\_m        &            &            & $-$*       & $+$*       &            & $-$*       &            &            & $-$        &            &            &            &            &            &             \\
&m            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$        & $+$        &            &            &            &            &            &            &             \\

\hline
\multicolumn{2}{l|}{\textbf{GNB}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            & $-$*       &            & $-$*       & $-$*       &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            & $-$*       & $+$*       &            & $-$*       &            &            &            &            &            &            &            &            &             \\
&m            & $+$*       & $+$*       &            & $+$*       & $+$*       &            &            &            &            &            &            &            &            &            &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            & $-$*       &            &            & $-$        &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            & $-$*       &            &            &            &            &            &            &            &            &            &            &            &             \\
&m            & $+$*       & $+$*       &            & $+$        &            &            &            &            &            &            &            &            &            &            &             \\

\hline
\multicolumn{2}{l|}{\textbf{MPR}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            & $-$*       &            &            &            &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            & $-$*       &            &            &            &            &            &            &            &            &            &            &            &             \\
&m            & $+$*       & $+$*       &            &            &            &            &            &            &            &            &            &            &            &            &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            & $-$*       &            & $-$*       & $-$*       &            & $-$        & $-$        &            &            & $-$        &            &            &             \\
&ip\_m        &            &            & $-$*       & $+$*       &            & $-$*       & $+$        &            &            &            &            &            &            &            &             \\
&m            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$        &            &            & $+$        &            &            &            &            &             \\

\hline
\multicolumn{2}{l|}{\textbf{RF}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            & $-$*       &            & $-$*       & $-$*       &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            & $-$*       & $+$*       &            & $-$        &            &            &            &            &            &            &            &            &             \\
&m            & $+$*       & $+$*       &            & $+$*       & $+$        &            &            &            &            &            &            &            &            &            &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            & $-$*       &            &            &            &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            & $-$*       &            &            &            &            &            &            &            &            &            &            &            &             \\
&m            & $+$*       & $+$*       &            &            &            &            &            &            &            &            &            &            &            &            &             \\

\hline
\multicolumn{2}{l|}{\textbf{QDA}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            & $-$*       &            &            & $+$*       &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            & $-$*       &            &            & $+$*       &            &            &            &            &            &            &            &            &             \\
&m            & $+$*       & $+$*       &            & $-$*       & $-$*       &            &            &            &            &            &            &            &            &            &             \\

\hline
\hline
\hline
\end{tabular}

  }
\end{table}

==> sections/2-cars-data/plots.tex <==
\begin{figure}[htbp]
\floatconts
  {fig:cars}
  {\caption{Results for \textit{cars}: \textit{M} - dashed line,
  \textit{IP} - dash and dot line, \textit{IP\_M} - thin solid line}}
  {%
    \subfigure[Distribution between classes]{
    \label{fig:cars:dist-class}%
    \includeteximage{plots/cars-dist-class}
    }%
    \qquad
    \subfigure[Baseline error, $b\_err$]{\label{fig:cars:baseline-error}%
      \includeteximage{plots/cars-baseline-error}
      }
    \qquad
    \subfigure[$oneC$: SVM and DT]{\label{fig:cars:oneC-SVM-DT}%
      \includeteximage{plots/cars-oneC-0}
      %\includeteximage{plots/cars-dist-class}
      }
    \qquad
    \subfigure[$avgC$: SVM and DT]{\label{fig:cars:avgC-SVM-DT}%
      \includeteximage{plots/cars-avgC-0}
      }
    \qquad
    \subfigure[$oneC$: KNN and Ada]{\label{fig:cars:oneC-KNN-Ada}%
      \includeteximage{plots/cars-oneC-2}
      }
    \qquad
    \subfigure[$avgC$: KNN and Ada]{\label{fig:cars:avgC-KNN-Ada}%
      \includeteximage{plots/cars-avgC-2}
      }
    \qquad
    \subfigure[$oneC$: GNB and MPR]{\label{fig:cars:oneC-GNB-MPR}%
      \includeteximage{plots/cars-oneC-4}
      }
    \qquad
    \subfigure[$avgC$: GNB and MPR]{\label{fig:cars:avgC-GNB-MPR}%
      \includeteximage{plots/cars-avgC-4}
      }
    \qquad
    \subfigure[$oneC$: RF and QDA]{\label{fig:cars:oneC-RF-QDA}%
      \includeteximage{plots/cars-oneC-6}
      }
    \qquad
    \subfigure[$avgC$: RF and QDA]{\label{fig:cars:avgC-RF-QDA}%
      \includeteximage{plots/cars-avgC-6}
      }
  }
\end{figure}


==> sections/2-cars-data/table_threshold.tex <==
\begin{table}[htbp]
\scriptsize
 % The first argument is the label.
 % The caption goes in the second argument, and the table contents
 % go in the third argument.
\floatconts
  {tab:cars}%
  {\caption{Significance of results for the \textit{cars} dataset}}%
  {
\begin{tabular}{cl|lll|lll|lll|lll|lll}
             && \multicolumn{3}{c|}{$\epsilon=0.01$} & \multicolumn{3}{c|}{$\epsilon=0.05$} & \multicolumn{3}{c|}{$\epsilon=0.1$} & \multicolumn{3}{c|}{$\epsilon=0.15$} & \multicolumn{3}{c}{$\epsilon=0.2$} \\
\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&m            &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\

\hline
\multicolumn{2}{l|}{\textbf{SVM}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            & $+$*       &            &            &            &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            & $+$*       &            &            &            &            &            &            &            &            &            &            &            &             \\
&m            & $-$*       & $-$*       &            &            &            &            &            &            &            &            &            &            &            &            &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            & $-$*       &            &            &            &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&m            & $+$*       &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\

\hline
\multicolumn{2}{l|}{\textbf{DT}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            & $+$*       &            &            &            &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            & $+$*       &            &            &            &            &            &            &            &            &            &            &            &             \\
&m            & $-$*       & $-$*       &            &            &            &            &            &            &            &            &            &            &            &            &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            &            & $-$*       &            & $-$        & $-$*       &            &            &             \\
&ip\_m        & $+$*       &            & $-$*       & $+$*       &            & $-$*       &            &            & $-$*       & $+$        &            & $-$*       &            &            &             \\
&m            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            &            &            &             \\

\hline
\multicolumn{2}{l|}{\textbf{KNN}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            & $-$        & $-$*       &            &            & $-$*       &            &            & $-$*       &            &            & $-$*       &            &            &             \\
&ip\_m        & $+$        &            & $-$*       &            &            & $-$*       &            &            & $-$*       &            &            & $-$*       &            &            &             \\
&m            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            &            &            &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            & $-$*       &            &            &            &            &            & $-$*       &            &            & $-$*       &            &            & $-$*        \\
&ip\_m        &            &            &            &            &            &            &            &            & $-$*       &            &            & $-$*       &            &            & $-$*        \\
&m            & $+$*       &            &            &            &            &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &             \\

\hline
\multicolumn{2}{l|}{\textbf{Ada}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            & $+$*       &            &            & $+$*       &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            & $+$*       &            &            & $+$*       &            &            &            &            &            &            &            &            &             \\
&m            & $-$*       & $-$*       &            & $-$*       & $-$*       &            &            &            &            &            &            &            &            &            &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            & $-$*       &            &            &            &            &            & $-$*       &            &            & $-$        &            &            & $-$         \\
&ip\_m        &            &            &            &            &            &            &            &            & $-$*       &            &            & $-$        &            &            & $-$         \\
&m            & $+$*       &            &            &            &            &            & $+$*       & $+$*       &            & $+$        & $+$        &            & $+$        & $+$        &             \\

\hline
\multicolumn{2}{l|}{\textbf{GNB}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            & $+$*       &            &            & $+$*       &            &            & $+$*       &            &            & $+$*       &            &            & $+$*        \\
&ip\_m        &            &            & $+$*       &            &            & $+$*       &            &            & $+$*       &            &            & $+$*       &            &            & $+$*        \\
&m            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            & $-$*       & $-$*       &            &            & $-$        &            &            & $-$*       &            &            &            &            &            &             \\
&ip\_m        & $+$*       &            & $-$        &            &            &            &            &            & $-$*       &            &            &            &            &            &             \\
&m            & $+$*       & $+$        &            & $+$        &            &            & $+$*       & $+$*       &            &            &            &            &            &            &             \\

\hline
\multicolumn{2}{l|}{\textbf{MPR}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            & $+$*       &            &            &            &            &            &            &            &            &            &            &            &             \\
&m            &            & $-$*       &            &            &            &            &            &            &            &            &            &            &            &            &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       &            &            & $-$*       & $-$*       &            &            & $-$*        \\
&ip\_m        & $+$*       &            & $-$*       & $+$*       &            &            & $+$*       &            & $+$*       & $+$*       &            & $-$*       &            &            & $-$*        \\
&m            & $+$*       & $+$*       &            & $+$*       &            &            &            & $-$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &             \\

\hline
\multicolumn{2}{l|}{\textbf{RF}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            & $-$*       &            &            & $-$*       &            &            & $-$*       &            &            &            &            &            &            &             \\
&ip\_m        & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       &            &            & $+$*       &            &            &             \\
&m            &            & $-$*       &            &            & $-$*       &            &            & $-$*       &            &            & $-$*       &            &            &            &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&m            &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\

\hline
\multicolumn{2}{l|}{\textbf{QDA}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&m            &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\

\hline
\hline
\hline
\end{tabular}

  }
\end{table}

==> sections/3-glass-data/plots.tex <==
\begin{figure}[htbp]
\floatconts
  {fig:glass}
  {\caption{Results for \textit{glass}: \textit{M} - dashed line,
  \textit{IP} - dash and dot line, \textit{IP\_M} - thin solid line}}
  {%
    \subfigure[Distribution between classes]{
    \label{fig:glass:dist-class}%
    \includeteximage{plots/glass-dist-class}
    }%
    \qquad
    \subfigure[Baseline error, $b\_err$]{\label{fig:glass:baseline-error}%
      \includeteximage{plots/glass-baseline-error}
      }
    \qquad
    \subfigure[$oneC$: SVM and DT]{\label{fig:glass:oneC-SVM-DT}%
      \includeteximage{plots/glass-oneC-0}
      %\includeteximage{plots/glass-dist-class}
      }
    \qquad
    \subfigure[$avgC$: SVM and DT]{\label{fig:glass:avgC-SVM-DT}%
      \includeteximage{plots/glass-avgC-0}
      }
    \qquad
    \subfigure[$oneC$: KNN and Ada]{\label{fig:glass:oneC-KNN-Ada}%
      \includeteximage{plots/glass-oneC-2}
      }
    \qquad
    \subfigure[$avgC$: KNN and Ada]{\label{fig:glass:avgC-KNN-Ada}%
      \includeteximage{plots/glass-avgC-2}
      }
    \qquad
    \subfigure[$oneC$: GNB and MPR]{\label{fig:glass:oneC-GNB-MPR}%
      \includeteximage{plots/glass-oneC-4}
      }
    \qquad
    \subfigure[$avgC$: GNB and MPR]{\label{fig:glass:avgC-GNB-MPR}%
      \includeteximage{plots/glass-avgC-4}
      }
    \qquad
    \subfigure[$oneC$: RF and QDA]{\label{fig:glass:oneC-RF-QDA}%
      \includeteximage{plots/glass-oneC-6}
      }
    \qquad
    \subfigure[$avgC$: RF and QDA]{\label{fig:glass:avgC-RF-QDA}%
      \includeteximage{plots/glass-avgC-6}
      }
  }
\end{figure}



==> sections/3-glass-data/table_threshold.tex <==
\begin{table}[htbp]
\scriptsize
 % The first argument is the label.
 % The caption goes in the second argument, and the table contents
 % go in the third argument.
\floatconts
  {tab:glass}%
  {\caption{Significance of results for the \textit{glass} dataset}}%
  {
\begin{tabular}{cl|lll|lll|lll|lll|lll}
             && \multicolumn{3}{c|}{$\epsilon=0.01$} & \multicolumn{3}{c|}{$\epsilon=0.05$} & \multicolumn{3}{c|}{$\epsilon=0.1$} & \multicolumn{3}{c|}{$\epsilon=0.15$} & \multicolumn{3}{c}{$\epsilon=0.2$} \\
\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            &            &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$        & $-$*       &            & $-$        & $-$*        \\
&ip\_m        &            &            &            & $+$*       &            & $-$*       & $+$*       &            & $-$        & $+$        &            & $-$        & $+$        &            & $-$         \\
&m            &            &            &            & $+$*       & $+$*       &            & $+$*       & $+$        &            & $+$*       & $+$        &            & $+$*       & $+$        &             \\

\hline
\multicolumn{2}{l|}{\textbf{SVM}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            &            &            &            & $+$*       &            &            & $+$        &            &            &            &            &            &             \\
&ip\_m        &            &            &            &            &            & $+$*       &            &            & $+$*       &            &            & $+$        &            &            &             \\
&m            &            &            &            & $-$*       & $-$*       &            & $-$        & $-$*       &            &            & $-$        &            &            &            &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            &            &            &            &            &            &            & $-$        &            & $-$        & $-$        &            & $-$        & $-$         \\
&ip\_m        &            &            &            &            &            &            &            &            & $-$        & $+$        &            & $-$        & $+$        &            & $-$         \\
&m            &            &            &            &            &            &            & $+$        & $+$        &            & $+$        & $+$        &            & $+$        & $+$        &             \\

\hline
\multicolumn{2}{l|}{\textbf{DT}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            &            &            &            &            &            &            & $-$        &            &            & $-$        &            &            & $-$         \\
&ip\_m        &            &            &            &            &            &            &            &            & $-$        &            &            & $-$        &            &            & $-$         \\
&m            &            &            &            &            &            &            & $+$        & $+$        &            & $+$        & $+$        &            & $+$        & $+$        &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            &            &            & $-$        & $-$*       &            & $-$        & $-$*       &            & $-$        & $-$*       &            & $-$        & $-$*        \\
&ip\_m        &            &            &            & $+$        &            & $-$        & $+$        &            & $-$        & $+$        &            & $-$*       & $+$        &            & $-$         \\
&m            &            &            &            & $+$*       & $+$        &            & $+$*       & $+$        &            & $+$*       & $+$*       &            & $+$*       & $+$        &             \\

\hline
\multicolumn{2}{l|}{\textbf{KNN}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            &            &            & $-$        & $-$        &            & $-$        & $-$        &            & $-$        & $-$        &            &            & $-$         \\
&ip\_m        &            &            &            & $+$        &            & $-$        & $+$        &            & $-$        & $+$        &            & $-$        &            &            &             \\
&m            &            &            &            & $+$        & $+$        &            & $+$        & $+$        &            & $+$        & $+$        &            & $+$        &            &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            &            &            &            &            &            &            & $-$*       &            &            & $-$*       &            & $-$*       & $-$*        \\
&ip\_m        &            &            &            &            &            &            &            &            & $-$        &            &            & $-$*       & $+$*       &            & $-$*        \\
&m            &            &            &            &            &            &            & $+$*       & $+$        &            & $+$*       & $+$*       &            & $+$*       & $+$*       &             \\

\hline
\multicolumn{2}{l|}{\textbf{Ada}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            &            &            &            & $+$*       &            &            & $+$*       &            &            & $+$*       &            &            & $+$*        \\
&ip\_m        &            &            &            &            &            & $+$*       &            &            & $+$*       &            &            & $+$*       &            &            & $+$*        \\
&m            &            &            &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            &            &            &            & $-$        &            & $-$        & $-$*       &            &            & $-$*       &            & $-$        & $-$*        \\
&ip\_m        &            &            &            &            &            &            & $+$        &            & $-$*       &            &            & $-$*       & $+$        &            & $-$*        \\
&m            &            &            &            & $+$        &            &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &             \\

\hline
\multicolumn{2}{l|}{\textbf{GNB}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            &            &            &            & $+$        &            &            & $+$*       &            &            & $+$*       &            &            & $+$*        \\
&ip\_m        &            &            &            &            &            & $+$        &            &            & $+$*       &            &            & $+$*       &            &            & $+$*        \\
&m            &            &            &            & $-$        & $-$        &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            &            &            & $-$        &            &            & $-$        & $-$        &            & $-$        &            &            & $-$        &             \\
&ip\_m        &            &            &            & $+$        &            & $+$        & $+$        &            & $+$        & $+$        &            & $+$        & $+$        &            & $+$         \\
&m            &            &            &            &            & $-$        &            & $+$        & $-$        &            &            & $-$        &            &            & $-$        &             \\

\hline
\multicolumn{2}{l|}{\textbf{MPR}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            &            &            &            & $+$*       &            & $-$        & $+$*       &            & $-$        & $+$*       &            & $-$        & $+$         \\
&ip\_m        &            &            &            &            &            & $+$*       & $+$        &            & $+$*       & $+$        &            & $+$*       & $+$        &            & $+$*        \\
&m            &            &            &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$        & $-$*       &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            &            &            & $-$        & $-$*       &            & $-$        & $-$*       &            & $-$        & $-$*       &            & $-$        & $-$*        \\
&ip\_m        &            &            &            & $+$        &            &            & $+$        &            & $-$        & $+$        &            & $-$        & $+$        &            & $-$         \\
&m            &            &            &            & $+$*       &            &            & $+$*       & $+$        &            & $+$*       & $+$        &            & $+$*       & $+$        &             \\

\hline
\multicolumn{2}{l|}{\textbf{RF}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            &            &            & $-$        & $+$        &            &            & $+$*       &            &            & $+$        &            &            &             \\
&ip\_m        &            &            &            & $+$        &            & $+$*       &            &            & $+$*       &            &            & $+$        &            &            &             \\
&m            &            &            &            & $-$        & $-$*       &            & $-$*       & $-$*       &            & $-$        & $-$        &            &            &            &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            &            &            &            & $-$*       &            &            & $-$*       &            &            & $-$        &            &            & $-$         \\
&ip\_m        &            &            &            &            &            & $-$*       &            &            & $-$        &            &            & $-$        &            &            &             \\
&m            &            &            &            & $+$*       & $+$*       &            & $+$*       & $+$        &            & $+$        & $+$        &            & $+$        &            &             \\

\hline
\multicolumn{2}{l|}{\textbf{QDA}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            &            &            &            &            &            &            & $-$        &            &            &            &            &            &             \\
&ip\_m        &            &            &            &            &            &            &            &            &            &            &            &            &            &            & $+$         \\
&m            &            &            &            &            &            &            & $+$        &            &            &            &            &            &            & $-$        &             \\

\hline
\hline
\hline
\end{tabular}

  }
\end{table}

==> sections/4-iris-data/plots.tex <==
\begin{figure}[htbp]
\floatconts
  {fig:iris}
  {\caption{Results for \textit{iris}: \textit{M} - dashed line,
  \textit{IP} - dash and dot line, \textit{IP\_M} - thin solid line}}
  {%
    \subfigure[Distribution between classes]{
    \label{fig:iris:dist-class}%
    \includeteximage{plots/iris-dist-class}
    }%
    \qquad
    \subfigure[Baseline error, $b\_err$]{\label{fig:iris:baseline-error}%
      \includeteximage{plots/iris-baseline-error}
      }
    \qquad
    \subfigure[$oneC$: SVM and DT]{\label{fig:iris:oneC-SVM-DT}%
      \includeteximage{plots/iris-oneC-0}
      %\includeteximage{plots/iris-dist-class}
      }
    \qquad
    \subfigure[$avgC$: SVM and DT]{\label{fig:iris:avgC-SVM-DT}%
      \includeteximage{plots/iris-avgC-0}
      }
    \qquad
    \subfigure[$oneC$: KNN and Ada]{\label{fig:iris:oneC-KNN-Ada}%
      \includeteximage{plots/iris-oneC-2}
      }
    \qquad
    \subfigure[$avgC$: KNN and Ada]{\label{fig:iris:avgC-KNN-Ada}%
      \includeteximage{plots/iris-avgC-2}
      }
    \qquad
    \subfigure[$oneC$: GNB and MPR]{\label{fig:iris:oneC-GNB-MPR}%
      \includeteximage{plots/iris-oneC-4}
      }
    \qquad
    \subfigure[$avgC$: GNB and MPR]{\label{fig:iris:avgC-GNB-MPR}%
      \includeteximage{plots/iris-avgC-4}
      }
    \qquad
    \subfigure[$oneC$: RF and QDA]{\label{fig:iris:oneC-RF-QDA}%
      \includeteximage{plots/iris-oneC-6}
      }
    \qquad
    \subfigure[$avgC$: RF and QDA]{\label{fig:iris:avgC-RF-QDA}%
      \includeteximage{plots/iris-avgC-6}
      }
  }
\end{figure}

==> sections/4-iris-data/table_threshold.tex <==
\begin{table}[htbp]
\scriptsize
 % The first argument is the label.
 % The caption goes in the second argument, and the table contents
 % go in the third argument.
\floatconts
  {tab:iris}%
  {\caption{Significance of results for the \textit{iris} dataset}}%
  {
\begin{tabular}{cl|lll|lll|lll|lll|lll}
             && \multicolumn{3}{c|}{$\epsilon=0.01$} & \multicolumn{3}{c|}{$\epsilon=0.05$} & \multicolumn{3}{c|}{$\epsilon=0.1$} & \multicolumn{3}{c|}{$\epsilon=0.15$} & \multicolumn{3}{c}{$\epsilon=0.2$} \\
\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&m            &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\

\hline
\multicolumn{2}{l|}{\textbf{SVM}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&m            &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&m            &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\

\hline
\multicolumn{2}{l|}{\textbf{DT}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&m            &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&m            &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\

\hline
\multicolumn{2}{l|}{\textbf{KNN}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&m            &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&m            &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\

\hline
\multicolumn{2}{l|}{\textbf{Ada}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            &            &            &            & $+$        &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            &            &            &            & $+$        &            &            &            &            &            &            &            &            &             \\
&m            &            &            &            & $-$        & $-$        &            &            &            &            &            &            &            &            &            &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&m            &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\

\hline
\multicolumn{2}{l|}{\textbf{GNB}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&m            &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&m            &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\

\hline
\multicolumn{2}{l|}{\textbf{MPR}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&m            &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            &            &            &            & $-$        &            &            & $-$        &            &            &            &            &            &             \\
&ip\_m        &            &            &            &            &            & $-$        &            &            &            &            &            &            &            &            &             \\
&m            &            &            &            & $+$        & $+$        &            & $+$        &            &            &            &            &            &            &            &             \\

\hline
\multicolumn{2}{l|}{\textbf{RF}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&m            &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&m            &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\

\hline
\multicolumn{2}{l|}{\textbf{QDA}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&m            &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\

\hline
\hline
\hline
\end{tabular}

  }
\end{table}

==> sections/5-user-data/plots.tex <==
\begin{figure}[htbp]
\floatconts
  {fig:user}
  {\caption{Results for \textit{user}: \textit{M} - dashed line,
  \textit{IP} - dash and dot line, \textit{IP\_M} - thin solid line}}
  {%
    \subfigure[Distribution between classes]{
    \label{fig:user:dist-class}%
    \includeteximage{plots/user-dist-class}
    }%
    \qquad
    \subfigure[Baseline error, $b\_err$]{\label{fig:user:baseline-error}%
      \includeteximage{plots/user-baseline-error}
      }
    \qquad
    \subfigure[$oneC$: SVM and DT]{\label{fig:user:oneC-SVM-DT}%
      \includeteximage{plots/user-oneC-0}
      %\includeteximage{plots/user-dist-class}
      }
    \qquad
    \subfigure[$avgC$: SVM and DT]{\label{fig:user:avgC-SVM-DT}%
      \includeteximage{plots/user-avgC-0}
      }
    \qquad
    \subfigure[$oneC$: KNN and Ada]{\label{fig:user:oneC-KNN-Ada}%
      \includeteximage{plots/user-oneC-2}
      }
    \qquad
    \subfigure[$avgC$: KNN and Ada]{\label{fig:user:avgC-KNN-Ada}%
      \includeteximage{plots/user-avgC-2}
      }
    \qquad
    \subfigure[$oneC$: GNB and MPR]{\label{fig:user:oneC-GNB-MPR}%
      \includeteximage{plots/user-oneC-4}
      }
    \qquad
    \subfigure[$avgC$: GNB and MPR]{\label{fig:user:avgC-GNB-MPR}%
      \includeteximage{plots/user-avgC-4}
      }
    \qquad
    \subfigure[$oneC$: RF and QDA]{\label{fig:user:oneC-RF-QDA}%
      \includeteximage{plots/user-oneC-6}
      }
    \qquad
    \subfigure[$avgC$: RF and QDA]{\label{fig:user:avgC-RF-QDA}%
      \includeteximage{plots/user-avgC-6}
      }
  }
\end{figure}

==> sections/5-user-data/table_threshold.tex <==
\begin{table}[htbp]
\scriptsize
 % The first argument is the label.
 % The caption goes in the second argument, and the table contents
 % go in the third argument.
\floatconts
  {tab:user}%
  {\caption{Significance of results for the \textit{user} dataset}}%
  {
\begin{tabular}{cl|lll|lll|lll|lll|lll}
             && \multicolumn{3}{c|}{$\epsilon=0.01$} & \multicolumn{3}{c|}{$\epsilon=0.05$} & \multicolumn{3}{c|}{$\epsilon=0.1$} & \multicolumn{3}{c|}{$\epsilon=0.15$} & \multicolumn{3}{c}{$\epsilon=0.2$} \\
\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&m            &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\

\hline
\multicolumn{2}{l|}{\textbf{SVM}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            &            &            &            & $+$*       &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            &            &            &            & $+$*       &            &            &            &            &            &            &            &            &             \\
&m            &            &            &            & $-$*       & $-$*       &            &            &            &            &            &            &            &            &            &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&m            &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\

\hline
\multicolumn{2}{l|}{\textbf{DT}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&m            &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            &            &            &            & $-$        &            &            & $-$*       &            &            & $-$        &            &            & $-$         \\
&ip\_m        &            &            &            &            &            & $-$        &            &            & $-$*       &            &            & $-$        &            &            & $-$         \\
&m            &            &            &            & $+$        & $+$        &            & $+$*       & $+$*       &            & $+$        & $+$        &            & $+$        & $+$        &             \\

\hline
\multicolumn{2}{l|}{\textbf{KNN}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            &            &            &            & $-$        &            &            & $-$*       &            &            &            &            &            &             \\
&ip\_m        &            &            &            &            &            & $-$        &            &            & $-$*       &            &            &            &            &            &             \\
&m            &            &            &            & $+$        & $+$        &            & $+$*       & $+$*       &            &            &            &            &            &            &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            &            &            &            &            &            &            &            &            &            & $+$        &            &            &             \\
&ip\_m        &            &            &            &            &            &            &            &            &            &            &            & $+$        &            &            &             \\
&m            &            &            &            &            &            &            &            &            &            & $-$        & $-$        &            &            &            &             \\

\hline
\multicolumn{2}{l|}{\textbf{Ada}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            &            &            &            & $+$*       &            &            & $+$*       &            &            & $+$*       &            &            & $+$         \\
&ip\_m        &            &            &            &            &            & $+$*       &            &            & $+$*       &            &            & $+$*       &            &            & $+$*        \\
&m            &            &            &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$        & $-$*       &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&m            &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\

\hline
\multicolumn{2}{l|}{\textbf{GNB}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            &            &            &            & $+$*       &            &            & $+$        &            &            &            &            &            &             \\
&ip\_m        &            &            &            &            &            & $+$*       &            &            & $+$        &            &            &            &            &            &             \\
&m            &            &            &            & $-$*       & $-$*       &            & $-$        & $-$        &            &            &            &            &            &            &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&m            &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\

\hline
\multicolumn{2}{l|}{\textbf{MPR}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&m            &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            &            &            & $-$        & $-$        &            & $-$*       &            &            &            &            &            &            &             \\
&ip\_m        &            &            &            & $+$        &            &            & $+$*       &            &            &            &            &            &            &            &             \\
&m            &            &            &            & $+$        &            &            &            &            &            &            &            &            &            &            &             \\

\hline
\multicolumn{2}{l|}{\textbf{RF}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            &            &            &            & $+$        &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            &            &            &            & $+$        &            &            &            &            &            &            &            &            &             \\
&m            &            &            &            & $-$        & $-$        &            &            &            &            &            &            &            &            &            &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&m            &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\

\hline
\multicolumn{2}{l|}{\textbf{QDA}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            &            &            &            & $+$        &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            &            &            &            & $+$        &            &            &            &            &            &            &            &            &             \\
&m            &            &            &            & $-$        & $-$        &            &            &            &            &            &            &            &            &            &             \\

\hline
\hline
\hline
\end{tabular}

  }
\end{table}

==> sections/6-wave-data/plots.tex <==
\begin{figure}[htbp]
\floatconts
  {fig:wave}
  {\caption{Results for \textit{wave}: \textit{M} - dashed line,
  \textit{IP} - dash and dot line, \textit{IP\_M} - thin solid line}}
  {%
    \subfigure[Distribution between classes]{
    \label{fig:wave:dist-class}%
    \includeteximage{plots/wave-dist-class}
    }%
    \qquad
    \subfigure[Baseline error, $b\_err$]{\label{fig:wave:baseline-error}%
      \includeteximage{plots/wave-baseline-error}
      }
    \qquad
    \subfigure[$oneC$: SVM and DT]{\label{fig:wave:oneC-SVM-DT}%
      \includeteximage{plots/wave-oneC-0}
      %\includeteximage{plots/wave-dist-class}
      }
    \qquad
    \subfigure[$avgC$: SVM and DT]{\label{fig:wave:avgC-SVM-DT}%
      \includeteximage{plots/wave-avgC-0}
      }
    \qquad
    \subfigure[$oneC$: KNN and Ada]{\label{fig:wave:oneC-KNN-Ada}%
      \includeteximage{plots/wave-oneC-2}
      }
    \qquad
    \subfigure[$avgC$: KNN and Ada]{\label{fig:wave:avgC-KNN-Ada}%
      \includeteximage{plots/wave-avgC-2}
      }
    \qquad
    \subfigure[$oneC$: GNB and MPR]{\label{fig:wave:oneC-GNB-MPR}%
      \includeteximage{plots/wave-oneC-4}
      }
    \qquad
    \subfigure[$avgC$: GNB and MPR]{\label{fig:wave:avgC-GNB-MPR}%
      \includeteximage{plots/wave-avgC-4}
      }
    \qquad
    \subfigure[$oneC$: RF and QDA]{\label{fig:wave:oneC-RF-QDA}%
      \includeteximage{plots/wave-oneC-6}
      }
    \qquad
    \subfigure[$avgC$: RF and QDA]{\label{fig:wave:avgC-RF-QDA}%
      \includeteximage{plots/wave-avgC-6}
      }
  }
\end{figure}




==> sections/6-wave-data/table_threshold.tex <==
\begin{table}[htbp]
\scriptsize
 % The first argument is the label.
 % The caption goes in the second argument, and the table contents
 % go in the third argument.
\floatconts
  {tab:wave}%
  {\caption{Significance of results for the \textit{wave} dataset}}%
  {
\begin{tabular}{cl|lll|lll|lll|lll|lll}
             && \multicolumn{3}{c|}{$\epsilon=0.01$} & \multicolumn{3}{c|}{$\epsilon=0.05$} & \multicolumn{3}{c|}{$\epsilon=0.1$} & \multicolumn{3}{c|}{$\epsilon=0.15$} & \multicolumn{3}{c}{$\epsilon=0.2$} \\
\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&m            &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\

\hline
\multicolumn{2}{l|}{\textbf{SVM}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            & $+$*       &            &            & $+$*       &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            & $+$*       &            &            & $+$*       &            &            &            &            &            &            &            &            &             \\
&m            & $-$*       & $-$*       &            & $-$*       & $-$*       &            &            &            &            &            &            &            &            &            &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            &            &            &            & $-$*       &            &            & $-$*       &            &            &            &            &            &             \\
&ip\_m        &            &            &            &            &            & $-$*       &            &            & $-$*       &            &            &            &            &            &             \\
&m            &            &            &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            &            &            &            &            &            &             \\

\hline
\multicolumn{2}{l|}{\textbf{DT}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            &            &            &            & $+$*       &            &            & $+$*       &            &            &            &            &            &             \\
&ip\_m        &            &            &            &            &            & $+$*       &            &            & $+$*       &            &            &            &            &            &             \\
&m            &            &            &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            &            &            &            &            &            &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&m            &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\

\hline
\multicolumn{2}{l|}{\textbf{KNN}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&m            &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            & $+$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*        \\
&ip\_m        &            &            & $+$*       & $+$*       &            &            & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*        \\
&m            & $-$*       & $-$*       &            & $+$*       &            &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &             \\

\hline
\multicolumn{2}{l|}{\textbf{Ada}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            & $+$*       &            & $-$*       &            &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*        \\
&ip\_m        &            &            & $+$*       & $+$*       &            &            & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*        \\
&m            & $-$*       & $-$*       &            &            &            &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&m            &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\

\hline
\multicolumn{2}{l|}{\textbf{GNB}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            & $+$*       &            &            & $+$*       &            &            & $+$*       &            &            &            &            &            &             \\
&ip\_m        &            &            & $+$*       &            &            & $+$*       &            &            & $+$*       &            &            &            &            &            &             \\
&m            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            &            &            &            &            &            &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&m            &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\

\hline
\multicolumn{2}{l|}{\textbf{MPR}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            & $+$*       &            &            &            &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            & $+$*       &            &            & $+$*       &            &            &            &            &            &            &            &            &             \\
&m            & $-$*       & $-$*       &            &            & $-$*       &            &            &            &            &            &            &            &            &            &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            & $-$*       &            &            & $-$*       &            &            & $-$*       &            &            & $-$*       & $-$*       &            & $-$*       & $-$*        \\
&ip\_m        & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*        \\
&m            &            & $-$*       &            &            & $-$*       &            &            & $-$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &             \\

\hline
\multicolumn{2}{l|}{\textbf{RF}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*       &            &            & $-$*       &            &            &            &             \\
&ip\_m        & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       &            &            &             \\
&m            & $-$*       & $-$*       &            & $-$*       & $-$*       &            &            & $-$*       &            &            & $-$*       &            &            &            &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&m            &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\

\hline
\multicolumn{2}{l|}{\textbf{QDA}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            & $+$*       &            &            &            &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            & $+$*       &            &            &            &            &            &            &            &            &            &            &            &             \\
&m            & $-$*       & $-$*       &            &            &            &            &            &            &            &            &            &            &            &            &             \\

\hline
\hline
\hline
\end{tabular}

  }
\end{table}

==> sections/7-wineR-data/plots.tex <==
\begin{figure}[htbp]
\floatconts
  {fig:wineRed}
  {\caption{Results for \textit{wineR}: \textit{M} - dashed line,
  \textit{IP} - dash and dot line, \textit{IP\_M} - thin solid line}}
  {%
    \subfigure[Distribution between classes]{
    \label{fig:wineRed:dist-class}%
    \includeteximage{plots/wine_Red-dist-class}
    }%
    \qquad
    \subfigure[Baseline error, $b\_err$]{\label{fig:wineRed:baseline-error}%
      \includeteximage{plots/wine_Red-baseline-error}
      }
    \qquad
    \subfigure[$oneC$: SVM and DT]{\label{fig:wineRed:oneC-SVM-DT}%
      \includeteximage{plots/wine_Red-oneC-0}
      %\includeteximage{plots/wine_Red-dist-class}
      }
    \qquad
    \subfigure[$avgC$: SVM and DT]{\label{fig:wineRed:avgC-SVM-DT}%
      \includeteximage{plots/wine_Red-avgC-0}
      }
    \qquad
    \subfigure[$oneC$: KNN and Ada]{\label{fig:wineRed:oneC-KNN-Ada}%
      \includeteximage{plots/wine_Red-oneC-2}
      }
    \qquad
    \subfigure[$avgC$: KNN and Ada]{\label{fig:wineRed:avgC-KNN-Ada}%
      \includeteximage{plots/wine_Red-avgC-2}
      }
    \qquad
    \subfigure[$oneC$: GNB and MPR]{\label{fig:wineRed:oneC-GNB-MPR}%
      \includeteximage{plots/wine_Red-oneC-4}
      }
    \qquad
    \subfigure[$avgC$: GNB and MPR]{\label{fig:wineRed:avgC-GNB-MPR}%
      \includeteximage{plots/wine_Red-avgC-4}
      }
    \qquad
    \subfigure[$oneC$: RF and QDA]{\label{fig:wineRed:oneC-RF-QDA}%
      \includeteximage{plots/wine_Red-oneC-6}
      }
    \qquad
    \subfigure[$avgC$: RF and QDA]{\label{fig:wineRed:avgC-RF-QDA}%
      \includeteximage{plots/wine_Red-avgC-6}
      }
  }
\end{figure}





==> sections/7-wineR-data/table_threshold.tex <==
\begin{table}[htbp]
\scriptsize
 % The first argument is the label.
 % The caption goes in the second argument, and the table contents
 % go in the third argument.
\floatconts
  {tab:wineR}%
  {\caption{Significance of results for the \textit{wineR} dataset}}%
  {
\begin{tabular}{cl|lll|lll|lll|lll|lll}
             && \multicolumn{3}{c|}{$\epsilon=0.01$} & \multicolumn{3}{c|}{$\epsilon=0.05$} & \multicolumn{3}{c|}{$\epsilon=0.1$} & \multicolumn{3}{c|}{$\epsilon=0.15$} & \multicolumn{3}{c}{$\epsilon=0.2$} \\
\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            &            &             \\
&ip\_m        & $+$*       &            &            & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*       &            &            &             \\
&m            & $+$*       &            &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            &            &            &             \\

\hline
\multicolumn{2}{l|}{\textbf{SVM}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            & $+$*       &            &            & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            &            & $+$*        \\
&ip\_m        &            &            & $+$*       &            &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       &            &            & $+$*        \\
&m            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            &            & $-$*       &            &            & $-$*        \\
&ip\_m        &            &            &            & $+$*       &            & $-$*       & $+$*       &            & $-$*       &            &            & $-$*       &            &            & $-$*        \\
&m            & $+$*       &            &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &             \\

\hline
\multicolumn{2}{l|}{\textbf{DT}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            &            &            & $-$        & $-$        &            &            & $+$*       &            &            & $+$*       &            &            & $+$*        \\
&ip\_m        &            &            &            & $+$        &            &            &            &            & $+$*       &            &            & $+$*       &            &            & $+$*        \\
&m            &            &            &            & $+$        &            &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            &            &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            &            & $-$*        \\
&ip\_m        &            &            &            & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            &            &            &            & $-$*        \\
&m            &            &            &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       &            &            & $+$*       & $+$*       &             \\

\hline
\multicolumn{2}{l|}{\textbf{KNN}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            &            &            &            & $-$*       &            & $-$*       & $-$*       &            &            &            &            &            & $+$*        \\
&ip\_m        &            &            &            &            &            & $-$*       & $+$*       &            & $-$*       &            &            &            &            &            & $+$*        \\
&m            &            &            &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            &            &            &            & $-$*       & $-$*       &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            &            &            &            &            &            &            &            &            &            & $+$*       &            &            &             \\
&m            &            &            &            &            &            &            &            &            &            &            & $-$*       &            &            &            &             \\

\hline
\multicolumn{2}{l|}{\textbf{Ada}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            & $+$*       &            &            &            &            &            & $-$*       &            &            & $-$*       &            &            & $-$*        \\
&ip\_m        &            &            & $+$*       &            &            &            &            &            & $-$*       &            &            & $-$*       &            &            & $-$*        \\
&m            & $-$*       & $-$*       &            &            &            &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            &            & $-$*       &            &            & $-$*        \\
&ip\_m        & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*       &            &            & $-$*       &            &            & $-$*        \\
&m            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &             \\

\hline
\multicolumn{2}{l|}{\textbf{GNB}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            & $+$        &            &            & $+$*       &            &            & $+$*       &            &            & $+$*       &            &            & $+$*        \\
&ip\_m        &            &            & $+$        &            &            & $+$*       &            &            & $+$*       &            &            & $+$*       &            &            & $+$*        \\
&m            & $-$        & $-$        &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$        & $-$         \\
&ip\_m        & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$        & $+$        &            &             \\
&m            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$        &            & $+$        &            &             \\

\hline
\multicolumn{2}{l|}{\textbf{MPR}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            & $+$*       &            &            & $+$*       &            &            & $+$*       &            & $-$*       & $+$*       &            &            & $+$*        \\
&ip\_m        &            &            & $+$*       &            &            & $+$*       &            &            & $+$*       & $+$*       &            & $+$*       &            &            & $+$*        \\
&m            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$         \\
&ip\_m        & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            &            & $+$*       &            &             \\
&m            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       &            &            & $+$        &            &             \\

\hline
\multicolumn{2}{l|}{\textbf{RF}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            & $+$*       &            &            & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*       &             \\
&ip\_m        &            &            & $+$*       &            &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*        \\
&m            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            &            & $-$*       &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            &            & $-$*       &            &            & $-$*        \\
&ip\_m        & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*       &            &            & $-$*       &            &            & $-$*        \\
&m            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &             \\

\hline
\multicolumn{2}{l|}{\textbf{QDA}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            &            &            &            & $+$*       &            &            & $+$*       &            &            & $+$*       &            &            & $+$*        \\
&ip\_m        &            &            &            &            &            & $+$*       &            &            & $+$*       &            &            & $+$*       &            &            & $+$*        \\
&m            &            &            &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &             \\

\hline
\hline
\hline
\end{tabular}

  }
\end{table}

==> sections/8-wineW-data/plots.tex <==


\begin{figure}[htbp]
\floatconts
  {fig:wineWhite}
  {\caption{Results for \textit{wineW}: \textit{M} - dashed line,
  \textit{IP} - dash and dot line, \textit{IP\_M} - thin solid line}}
  {%
    \subfigure[Distribution between classes]{
    \label{fig:wineWhite:dist-class}%
    \includeteximage{plots/wine_White-dist-class}
    }%
    \qquad
    \subfigure[Baseline error, $b\_err$]{\label{fig:wineWhite:baseline-error}%
      \includeteximage{plots/wine_White-baseline-error}
      }
    \qquad
    \subfigure[$oneC$: SVM and DT]{\label{fig:wineWhite:oneC-SVM-DT}%
      \includeteximage{plots/wine_White-oneC-0}
      %\includeteximage{plots/wine_White-dist-class}
      }
    \qquad
    \subfigure[$avgC$: SVM and DT]{\label{fig:wineWhite:avgC-SVM-DT}%
      \includeteximage{plots/wine_White-avgC-0}
      }
    \qquad
    \subfigure[$oneC$: KNN and Ada]{\label{fig:wineWhite:oneC-KNN-Ada}%
      \includeteximage{plots/wine_White-oneC-2}
      }
    \qquad
    \subfigure[$avgC$: KNN and Ada]{\label{fig:wineWhite:avgC-KNN-Ada}%
      \includeteximage{plots/wine_White-avgC-2}
      }
    \qquad
    \subfigure[$oneC$: GNB and MPR]{\label{fig:wineWhite:oneC-GNB-MPR}%
      \includeteximage{plots/wine_White-oneC-4}
      }
    \qquad
    \subfigure[$avgC$: GNB and MPR]{\label{fig:wineWhite:avgC-GNB-MPR}%
      \includeteximage{plots/wine_White-avgC-4}
      }
    \qquad
    \subfigure[$oneC$: RF and QDA]{\label{fig:wineWhite:oneC-RF-QDA}%
      \includeteximage{plots/wine_White-oneC-6}
      }
    \qquad
    \subfigure[$avgC$: RF and QDA]{\label{fig:wineWhite:avgC-RF-QDA}%
      \includeteximage{plots/wine_White-avgC-6}
      }
  }
\end{figure}



==> sections/8-wineW-data/table_threshold.tex <==
\begin{table}[htbp]
\scriptsize
 % The first argument is the label.
 % The caption goes in the second argument, and the table contents
 % go in the third argument.
\floatconts
  {tab:wineW}%
  {\caption{Significance of results for the \textit{wineW} dataset}}%
  {
\begin{tabular}{cl|lll|lll|lll|lll|lll}
             && \multicolumn{3}{c|}{$\epsilon=0.01$} & \multicolumn{3}{c|}{$\epsilon=0.05$} & \multicolumn{3}{c|}{$\epsilon=0.1$} & \multicolumn{3}{c|}{$\epsilon=0.15$} & \multicolumn{3}{c}{$\epsilon=0.2$} \\
\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            &            & $-$*       &            &            & $-$*        \\
&ip\_m        & $+$*       &            &            & $+$*       &            & $-$*       & $+$*       &            & $-$*       &            &            & $-$*       &            &            & $-$*        \\
&m            & $+$*       &            &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &             \\

\hline
\multicolumn{2}{l|}{\textbf{SVM}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            & $+$*       &            &            & $+$*       &            &            &            &            &            & $+$*       &            &            & $+$*        \\
&ip\_m        &            &            & $+$*       &            &            & $+$*       &            &            &            &            &            & $+$*       &            &            & $+$*        \\
&m            & $-$*       & $-$*       &            & $-$*       & $-$*       &            &            &            &            & $-$*       & $-$*       &            & $-$*       & $-$*       &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            &            & $-$*        \\
&ip\_m        & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*       &            &            & $-$*        \\
&m            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &             \\

\hline
\multicolumn{2}{l|}{\textbf{DT}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            &            &            &            & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            &            & $+$*        \\
&ip\_m        &            &            &            &            &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       &            &            & $+$*        \\
&m            &            &            &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            &            &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            &            & $-$*        \\
&ip\_m        &            &            &            & $+$*       &            & $-$*       & $+$*       &            &            & $+$*       &            &            &            &            & $-$*        \\
&m            &            &            &            & $+$*       & $+$*       &            & $+$*       &            &            & $+$*       &            &            & $+$*       & $+$*       &             \\

\hline
\multicolumn{2}{l|}{\textbf{KNN}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            &            &            & $-$        & $-$*       &            & $-$*       & $-$*       &            &            &            &            &            & $+$*        \\
&ip\_m        &            &            &            & $+$        &            & $-$        & $+$*       &            & $-$*       &            &            & $+$        &            &            & $+$*        \\
&m            &            &            &            & $+$*       & $+$        &            & $+$*       & $+$*       &            &            & $-$        &            & $-$*       & $-$*       &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&m            &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\

\hline
\multicolumn{2}{l|}{\textbf{Ada}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            & $+$        &            &            &            &            &            &            &            &            &            &            &            & $-$         \\
&ip\_m        &            &            & $+$        &            &            &            &            &            &            &            &            &            &            &            & $-$         \\
&m            & $-$        & $-$        &            &            &            &            &            &            &            &            &            &            & $+$        & $+$        &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*        \\
&ip\_m        & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*        \\
&m            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &             \\

\hline
\multicolumn{2}{l|}{\textbf{GNB}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            & $+$*       &            &            & $+$*       &            &            & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*        \\
&ip\_m        &            &            & $+$*       &            &            & $+$*       &            &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*        \\
&m            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*        \\
&ip\_m        & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            &             \\
&m            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       &            &             \\

\hline
\multicolumn{2}{l|}{\textbf{MPR}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            & $+$*       &            &            & $+$*       &            &            & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*        \\
&ip\_m        &            &            & $+$*       &            &            & $+$*       &            &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*        \\
&m            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*        \\
&ip\_m        & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$         \\
&m            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$        &             \\

\hline
\multicolumn{2}{l|}{\textbf{RF}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            & $+$*       &            &            & $+$*       &            &            & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*        \\
&ip\_m        &            &            & $+$*       &            &            & $+$*       &            &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*        \\
&m            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            &            & $-$*        \\
&ip\_m        & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*       &            &            & $-$*        \\
&m            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &             \\

\hline
\multicolumn{2}{l|}{\textbf{QDA}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            & $+$*       &            &            & $+$*       &            &            & $+$*       &            &            & $+$*       &            &            & $+$*        \\
&ip\_m        &            &            & $+$*       &            &            & $+$*       &            &            & $+$*       &            &            & $+$*       &            &            & $+$*        \\
&m            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &             \\

\hline
\hline
\hline
\end{tabular}

  }
\end{table}

==> sections/9-yeast-data/plots.tex <==


\begin{figure}[htbp]
\floatconts
  {fig:yeast}
  {\caption{Results for \textit{yeast}: \textit{M} - dashed line,
  \textit{IP} - dash and dot line, \textit{IP\_M} - thin solid line.}}
  {%
    \subfigure[Distribution between classes]{
    \label{fig:yeast:dist-class}%
    \includeteximage{plots/yeast-dist-class}
    }%
    \qquad
    \subfigure[Baseline error, $b\_err$]{\label{fig:yeast:baseline-error}%
      \includeteximage{plots/yeast-baseline-error}
      }
    \qquad
    \subfigure[$oneC$: SVM and DT]{\label{fig:yeast:oneC-SVM-DT}%
      \includeteximage{plots/yeast-oneC-0}
      %\includeteximage{plots/yeast-dist-class}
      }
    \qquad
    \subfigure[$avgC$: SVM and DT]{\label{fig:yeast:avgC-SVM-DT}%
      \includeteximage{plots/yeast-avgC-0}
      }
    \qquad
    \subfigure[$oneC$: KNN and Ada]{\label{fig:yeast:oneC-KNN-Ada}%
      \includeteximage{plots/yeast-oneC-2}
      }
    \qquad
    \subfigure[$avgC$: KNN and Ada]{\label{fig:yeast:avgC-KNN-Ada}%
      \includeteximage{plots/yeast-avgC-2}
      }
    \qquad
    \subfigure[$oneC$: GNB and MPR]{\label{fig:yeast:oneC-GNB-MPR}%
      \includeteximage{plots/yeast-oneC-4}
      }
    \qquad
    \subfigure[$avgC$: GNB and MPR]{\label{fig:yeast:avgC-GNB-MPR}%
      \includeteximage{plots/yeast-avgC-4}
      }
    \qquad
    \subfigure[$oneC$: RF and QDA]{\label{fig:yeast:oneC-RF-QDA}%
      \includeteximage{plots/yeast-oneC-6}
      }
    \qquad
    \subfigure[$avgC$: RF and QDA]{\label{fig:yeast:avgC-RF-QDA}%
      \includeteximage{plots/yeast-avgC-6}
      }
  }
\end{figure}




==> sections/9-yeast-data/table_threshold.tex <==
\begin{table}[htbp]
\scriptsize
 % The first argument is the label.
 % The caption goes in the second argument, and the table contents
 % go in the third argument.
\floatconts
  {tab:yeast}%
  {\caption{Significance of results for \textit{yeast} dataset}}%
  {
\begin{tabular}{cl|lll|lll|lll|lll|lll}
             && \multicolumn{3}{c|}{$\epsilon=0.01$} & \multicolumn{3}{c|}{$\epsilon=0.05$} & \multicolumn{3}{c|}{$\epsilon=0.1$} & \multicolumn{3}{c|}{$\epsilon=0.15$} & \multicolumn{3}{c}{$\epsilon=0.2$} \\
\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            &            & $-$*        \\
&ip\_m        & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*       &            &            & $-$*        \\
&m            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &             \\

\hline
\multicolumn{2}{l|}{\textbf{SVM}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            & $+$*       &            &            & $+$*       &            &            & $+$*       &            &            & $+$*       &            &            & $+$*        \\
&ip\_m        &            &            & $+$*       &            &            & $+$*       &            &            & $+$*       &            &            & $+$*       &            &            & $+$*        \\
&m            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            &            &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$        & $-$*        \\
&ip\_m        &            &            &            & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$        &            & $-$*        \\
&m            &            &            &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &             \\

\hline
\multicolumn{2}{l|}{\textbf{DT}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            &            &            & $-$*       & $-$*       &            & $-$        &            &            &            & $+$*       &            &            & $+$*        \\
&ip\_m        &            &            &            & $+$*       &            & $-$*       & $+$        &            & $+$        &            &            & $+$*       &            &            & $+$*        \\
&m            &            &            &            & $+$*       & $+$*       &            &            & $-$        &            & $-$*       & $-$*       &            & $-$*       & $-$*       &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            &            &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            &            & $-$*        \\
&ip\_m        &            &            &            & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*       &            &            & $-$*        \\
&m            &            &            &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &             \\

\hline
\multicolumn{2}{l|}{\textbf{KNN}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            &            &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$        & $-$*       &            &            & $+$*        \\
&ip\_m        &            &            &            & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$        &            & $-$*       &            &            & $+$*        \\
&m            &            &            &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $-$*       & $-$*       &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            & $-$*       &            &            & $-$*       &            &            &            &            & $-$        & $-$        &            & $-$*       & $-$*        \\
&ip\_m        &            &            &            &            &            &            &            &            &            & $+$        &            &            & $+$*       &            & $-$*        \\
&m            & $+$*       &            &            & $+$*       &            &            &            &            &            & $+$        &            &            & $+$*       & $+$*       &             \\

\hline
\multicolumn{2}{l|}{\textbf{Ada}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            & $+$*       &            &            & $+$*       &            &            &            &            &            & $-$*       &            &            & $-$*        \\
&ip\_m        &            &            & $+$*       &            &            & $+$*       &            &            &            &            &            & $-$        &            &            & $-$*        \\
&m            & $-$*       & $-$*       &            & $-$*       & $-$*       &            &            &            &            & $+$*       & $+$        &            & $+$*       & $+$*       &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*        \\
&ip\_m        & $+$*       &            &            & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*        \\
&m            & $+$*       &            &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &             \\

\hline
\multicolumn{2}{l|}{\textbf{GNB}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            &            &            &            & $+$*       &            & $-$        & $+$*       &            & $-$        & $+$*       &            & $-$        & $+$*        \\
&ip\_m        &            &            &            &            &            & $+$*       & $+$        &            & $+$*       & $+$        &            & $+$*       & $+$        &            & $+$*        \\
&m            &            &            &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*        \\
&ip\_m        & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*        \\
&m            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &             \\

\hline
\multicolumn{2}{l|}{\textbf{MPR}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            & $+$*       &            &            & $+$*       &            &            & $+$*       &            &            & $+$*       &            &            & $+$*        \\
&ip\_m        &            &            & $+$*       &            &            & $+$*       &            &            & $+$*       &            &            & $+$*       &            &            & $+$*        \\
&m            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*        \\
&ip\_m        & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*        \\
&m            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &             \\

\hline
\multicolumn{2}{l|}{\textbf{RF}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            & $+$*       &            &            & $+$*       &            &            & $+$*       &            &            & $+$*       &            &            & $+$*        \\
&ip\_m        &            &            & $+$*       &            &            & $+$*       &            &            & $+$*       &            &            & $+$*       &            &            & $+$*        \\
&m            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            &            &            &            &            &            &            & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*        \\
&ip\_m        &            &            &            &            &            &            &            &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*        \\
&m            &            &            &            &            &            &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &             \\

\hline
\multicolumn{2}{l|}{\textbf{QDA}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            &            &            &            &            &            &            &            &            &            & $-$*       &            &            & $-$*        \\
&ip\_m        &            &            &            &            &            &            &            &            &            &            &            & $-$*       &            &            & $-$*        \\
&m            &            &            &            &            &            &            &            &            &            & $+$*       & $+$*       &            & $+$*       & $+$*       &             \\

\hline
\hline
\hline
\end{tabular}

  }
\end{table}

==> sections/gen-05-data/plots.tex <==


\begin{figure}[htbp]
\floatconts
  {fig:gen-05}
  {\caption{$\sigma = 0.5$: \textit{M} - dashed line,
  \textit{IP} - dash and dot line, \textit{IP\_M} - thin solid line.}}
  {%
    \subfigure[Visualization of 4 classes]{
    \label{fig:gen-05:dist-class}%
    \includeteximage{plots/gen-05-class-visualization-partial}
    }%
    \qquad
    \subfigure[Baseline error, $b\_err$]{\label{fig:gen-05:baseline-error}%
      \includeteximage{plots/gen-05-baseline-error}
      }
    \qquad
    \subfigure[$oneC$: SVM and DT]{\label{fig:gen-05:oneC-SVM-DT}%
      \includeteximage{plots/gen-05-oneC-0}
      %\includeteximage{plots/gen-05-dist-class}
      }
    \qquad
    \subfigure[$avgC$: SVM and DT]{\label{fig:gen-05:avgC-SVM-DT}%
      \includeteximage{plots/gen-05-avgC-0}
      }
    \qquad
    \subfigure[$oneC$: KNN and Ada]{\label{fig:gen-05:oneC-KNN-Ada}%
      \includeteximage{plots/gen-05-oneC-2}
      }
    \qquad
    \subfigure[$avgC$: KNN and Ada]{\label{fig:gen-05:avgC-KNN-Ada}%
      \includeteximage{plots/gen-05-avgC-2}
      }
    \qquad
    \subfigure[$oneC$: GNB and MPR]{\label{fig:gen-05:oneC-GNB-MPR}%
      \includeteximage{plots/gen-05-oneC-4}
      }
    \qquad
    \subfigure[$avgC$: GNB and MPR]{\label{fig:gen-05:avgC-GNB-MPR}%
      \includeteximage{plots/gen-05-avgC-4}
      }
    \qquad
    \subfigure[$oneC$: RF and QDA]{\label{fig:gen-05:oneC-RF-QDA}%
      \includeteximage{plots/gen-05-oneC-6}
      }
    \qquad
    \subfigure[$avgC$: RF and QDA]{\label{fig:gen-05:avgC-RF-QDA}%
      \includeteximage{plots/gen-05-avgC-6}
      }
  }
\end{figure}




==> sections/gen-05-data/table_threshold.tex <==
\begin{table}[htbp]
\scriptsize
 % The first argument is the label.
 % The caption goes in the second argument, and the table contents
 % go in the third argument.
\floatconts
  {tab:gen_0.5}%
  {\caption{Significance of results for $\sigma = 0.5$}}%
  {
\begin{tabular}{cl|lll|lll|lll|lll|lll}
             && \multicolumn{3}{c|}{$\epsilon=0.01$} & \multicolumn{3}{c|}{$\epsilon=0.05$} & \multicolumn{3}{c|}{$\epsilon=0.1$} & \multicolumn{3}{c|}{$\epsilon=0.15$} & \multicolumn{3}{c}{$\epsilon=0.2$} \\
\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&m            &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\

\hline
\multicolumn{2}{l|}{\textbf{SVM}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&m            &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&m            &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\

\hline
\multicolumn{2}{l|}{\textbf{DT}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&m            &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&m            &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\

\hline
\multicolumn{2}{l|}{\textbf{KNN}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&m            &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&m            &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\

\hline
\multicolumn{2}{l|}{\textbf{Ada}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&m            &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&m            &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\

\hline
\multicolumn{2}{l|}{\textbf{GNB}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&m            &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&m            &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\

\hline
\multicolumn{2}{l|}{\textbf{MPR}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&m            &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&m            &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\

\hline
\multicolumn{2}{l|}{\textbf{RF}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&m            &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&m            &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\

\hline
\multicolumn{2}{l|}{\textbf{QDA}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&m            &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\

\hline
\hline
\hline
\end{tabular}

  }
\end{table}

==> sections/gen-075-data/plots.tex <==


\begin{figure}[htbp]
\floatconts
  {fig:gen-075}
  {\caption{$\sigma = 0.75$: \textit{M} - dashed line,
  \textit{IP} - dash and dot line, \textit{IP\_M} - thin solid line.}}
  {%
    \subfigure[Visualization of 4 classes]{
    \label{fig:gen-075:dist-class}%
    \includeteximage{plots/gen-075-class-visualization-partial}
    }%
    \qquad
    \subfigure[Baseline error, $b\_err$]{\label{fig:gen-075:baseline-error}%
      \includeteximage{plots/gen-075-baseline-error}
      }
    \qquad
    \subfigure[$oneC$: SVM and DT]{\label{fig:gen-075:oneC-SVM-DT}%
      \includeteximage{plots/gen-075-oneC-0}
      %\includeteximage{plots/gen-075-dist-class}
      }
    \qquad
    \subfigure[$avgC$: SVM and DT]{\label{fig:gen-075:avgC-SVM-DT}%
      \includeteximage{plots/gen-075-avgC-0}
      }
    \qquad
    \subfigure[$oneC$: KNN and Ada]{\label{fig:gen-075:oneC-KNN-Ada}%
      \includeteximage{plots/gen-075-oneC-2}
      }
    \qquad
    \subfigure[$avgC$: KNN and Ada]{\label{fig:gen-075:avgC-KNN-Ada}%
      \includeteximage{plots/gen-075-avgC-2}
      }
    \qquad
    \subfigure[$oneC$: GNB and MPR]{\label{fig:gen-075:oneC-GNB-MPR}%
      \includeteximage{plots/gen-075-oneC-4}
      }
    \qquad
    \subfigure[$avgC$: GNB and MPR]{\label{fig:gen-075:avgC-GNB-MPR}%
      \includeteximage{plots/gen-075-avgC-4}
      }
    \qquad
    \subfigure[$oneC$: RF and QDA]{\label{fig:gen-075:oneC-RF-QDA}%
      \includeteximage{plots/gen-075-oneC-6}
      }
    \qquad
    \subfigure[$avgC$: RF and QDA]{\label{fig:gen-075:avgC-RF-QDA}%
      \includeteximage{plots/gen-075-avgC-6}
      }
  }
\end{figure}




==> sections/gen-075-data/table_threshold.tex <==
\begin{table}[htbp]
\scriptsize
 % The first argument is the label.
 % The caption goes in the second argument, and the table contents
 % go in the third argument.
\floatconts
  {tab:gen_0.75}%
  {\caption{Significance of results for $\sigma = 0.75$}}%
  {
\begin{tabular}{cl|lll|lll|lll|lll|lll}
             && \multicolumn{3}{c|}{$\epsilon=0.01$} & \multicolumn{3}{c|}{$\epsilon=0.05$} & \multicolumn{3}{c|}{$\epsilon=0.1$} & \multicolumn{3}{c|}{$\epsilon=0.15$} & \multicolumn{3}{c}{$\epsilon=0.2$} \\
\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&m            &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\

\hline
\multicolumn{2}{l|}{\textbf{SVM}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            & $+$*       &            &            & $+$*       &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            & $+$*       &            &            & $+$*       &            &            &            &            &            &            &            &            &             \\
&m            & $-$*       & $-$*       &            & $-$*       & $-$*       &            &            &            &            &            &            &            &            &            &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&m            &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\

\hline
\multicolumn{2}{l|}{\textbf{DT}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            & $+$*       &            &            &            &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            & $+$*       &            &            &            &            &            &            &            &            &            &            &            &             \\
&m            & $-$*       & $-$*       &            &            &            &            &            &            &            &            &            &            &            &            &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&m            &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\

\hline
\multicolumn{2}{l|}{\textbf{KNN}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&m            &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&m            &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\

\hline
\multicolumn{2}{l|}{\textbf{Ada}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            & $+$*       &            &            &            &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            & $+$*       &            &            &            &            &            &            &            &            &            &            &            &             \\
&m            & $-$*       & $-$*       &            &            &            &            &            &            &            &            &            &            &            &            &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&m            &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\

\hline
\multicolumn{2}{l|}{\textbf{GNB}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            & $+$*       &            &            &            &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            & $+$*       &            &            &            &            &            &            &            &            &            &            &            &             \\
&m            & $-$*       & $-$*       &            &            &            &            &            &            &            &            &            &            &            &            &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&m            &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\

\hline
\multicolumn{2}{l|}{\textbf{MPR}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            & $+$*       &            &            &            &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            & $+$*       &            &            &            &            &            &            &            &            &            &            &            &             \\
&m            & $-$*       & $-$*       &            &            &            &            &            &            &            &            &            &            &            &            &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            & $-$*       &            &            & $-$*       &            &            & $-$*       & $-$*       &            &            &            &            &            &             \\
&ip\_m        & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            &            &            &            &            &            &            &             \\
&m            &            & $-$*       &            &            & $-$*       &            & $+$*       &            &            &            &            &            &            &            &             \\

\hline
\multicolumn{2}{l|}{\textbf{RF}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            & $-$*       &            &            & $-$*       &            &            & $-$*       &            &            &            &            &            &            &             \\
&ip\_m        & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       &            &            &            &            &            &             \\
&m            &            & $-$*       &            &            & $-$*       &            &            & $-$*       &            &            &            &            &            &            &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&m            &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\

\hline
\multicolumn{2}{l|}{\textbf{QDA}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            & $+$*       &            &            &            &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            & $+$*       &            &            &            &            &            &            &            &            &            &            &            &             \\
&m            & $-$*       & $-$*       &            &            &            &            &            &            &            &            &            &            &            &            &             \\

\hline
\hline
\hline
\end{tabular}

  }
\end{table}

==> sections/gen-1-data/plots.tex <==


\begin{figure}[htbp]
\floatconts
  {fig:gen-1}
  {\caption{$\sigma = 1$: \textit{M} - dashed line,
  \textit{IP} - dash and dot line, \textit{IP\_M} - thin solid line.}}
  {%
    \subfigure[Visualization of 4 classes]{
    \label{fig:gen-1:dist-class}%
    \includeteximage{plots/gen-1-class-visualization-partial}
    }%
    \qquad
    \subfigure[Baseline error, $b\_err$]{\label{fig:gen-1:baseline-error}%
      \includeteximage{plots/gen-1-baseline-error}
      }
    \qquad
    \subfigure[$oneC$: SVM and DT]{\label{fig:gen-1:oneC-SVM-DT}%
      \includeteximage{plots/gen-1-oneC-0}
      %\includeteximage{plots/gen-1-dist-class}
      }
    \qquad
    \subfigure[$avgC$: SVM and DT]{\label{fig:gen-1:avgC-SVM-DT}%
      \includeteximage{plots/gen-1-avgC-0}
      }
    \qquad
    \subfigure[$oneC$: KNN and Ada]{\label{fig:gen-1:oneC-KNN-Ada}%
      \includeteximage{plots/gen-1-oneC-2}
      }
    \qquad
    \subfigure[$avgC$: KNN and Ada]{\label{fig:gen-1:avgC-KNN-Ada}%
      \includeteximage{plots/gen-1-avgC-2}
      }
    \qquad
    \subfigure[$oneC$: GNB and MPR]{\label{fig:gen-1:oneC-GNB-MPR}%
      \includeteximage{plots/gen-1-oneC-4}
      }
    \qquad
    \subfigure[$avgC$: GNB and MPR]{\label{fig:gen-1:avgC-GNB-MPR}%
      \includeteximage{plots/gen-1-avgC-4}
      }
    \qquad
    \subfigure[$oneC$: RF and QDA]{\label{fig:gen-1:oneC-RF-QDA}%
      \includeteximage{plots/gen-1-oneC-6}
      }
    \qquad
    \subfigure[$avgC$: RF and QDA]{\label{fig:gen-1:avgC-RF-QDA}%
      \includeteximage{plots/gen-1-avgC-6}
      }
  }
\end{figure}




==> sections/gen-1-data/table_threshold.tex <==
\begin{table}[htbp]
\scriptsize
 % The first argument is the label.
 % The caption goes in the second argument, and the table contents
 % go in the third argument.
\floatconts
  {tab:gen_1}%
  {\caption{Significance of results for $\sigma = 1$}}%
  {
\begin{tabular}{cl|lll|lll|lll|lll|lll}
             && \multicolumn{3}{c|}{$\epsilon=0.01$} & \multicolumn{3}{c|}{$\epsilon=0.05$} & \multicolumn{3}{c|}{$\epsilon=0.1$} & \multicolumn{3}{c|}{$\epsilon=0.15$} & \multicolumn{3}{c}{$\epsilon=0.2$} \\
\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            & $-$*       & $-$*       &            &            &            &            &            &            &            &            &            &            &            &             \\
&ip\_m        & $+$*       &            & $-$*       &            &            &            &            &            &            &            &            &            &            &            &             \\
&m            & $+$*       & $+$*       &            &            &            &            &            &            &            &            &            &            &            &            &             \\

\hline
\multicolumn{2}{l|}{\textbf{SVM}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            & $-$*       & $+$*       &            &            & $+$*       &            &            & $+$*       &            &            & $+$*       &            &            &             \\
&ip\_m        & $+$*       &            & $+$*       &            &            & $+$*       &            &            & $+$*       &            &            & $+$*       &            &            &             \\
&m            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            &            &            &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&m            &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\

\hline
\multicolumn{2}{l|}{\textbf{DT}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            & $+$*       &            &            &            &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            & $+$*       &            &            &            &            &            &            &            &            &            &            &            &             \\
&m            & $-$*       & $-$*       &            &            &            &            &            &            &            &            &            &            &            &            &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            &            &            &            &            &            &            & $-$*       &            &            &            &            &            &             \\
&ip\_m        &            &            &            &            &            &            &            &            & $-$*       &            &            &            &            &            &             \\
&m            &            &            &            &            &            &            & $+$*       & $+$*       &            &            &            &            &            &            &             \\

\hline
\multicolumn{2}{l|}{\textbf{KNN}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            &            &            &            & $+$*       &            &            & $-$*       &            &            &            &            &            &             \\
&ip\_m        &            &            &            &            &            & $+$*       &            &            & $-$*       &            &            &            &            &            &             \\
&m            &            &            &            & $-$*       & $-$*       &            & $+$*       & $+$*       &            &            &            &            &            &            &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&m            &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\

\hline
\multicolumn{2}{l|}{\textbf{Ada}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&m            &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            & $-$*       & $-$*       &            &            & $-$*       &            &            & $-$*       &            &            & $-$*       &            &            & $-$*        \\
&ip\_m        & $+$*       &            & $-$*       &            &            & $-$*       &            &            & $-$*       &            &            & $-$*       &            &            & $-$*        \\
&m            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &             \\

\hline
\multicolumn{2}{l|}{\textbf{GNB}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            & $-$*       & $+$*       &            &            & $+$*       &            &            & $+$*       &            &            & $+$*       &            &            &             \\
&ip\_m        & $+$*       &            & $+$*       &            &            & $+$*       &            &            & $+$*       &            &            & $+$*       &            &            &             \\
&m            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            &            &            &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            & $-$*       & $-$*       &            &            & $-$*       &            &            & $-$*       &            &            & $-$*       &            &            & $-$*        \\
&ip\_m        & $+$*       &            & $-$*       &            &            & $-$*       &            &            & $-$*       &            &            & $-$*       &            &            & $-$*        \\
&m            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &             \\

\hline
\multicolumn{2}{l|}{\textbf{MPR}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            & $-$*       & $+$*       &            &            & $+$*       &            &            & $+$*       &            &            & $+$*       &            &            &             \\
&ip\_m        & $+$*       &            & $+$*       &            &            & $+$*       &            &            & $+$*       &            &            & $+$*       &            &            &             \\
&m            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            &            &            &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            & $-$*       &            &            & $-$*       &            &            & $-$*       &            &            & $-$*       &            &            & $-$*       & $-$*        \\
&ip\_m        & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            &             \\
&m            &            & $-$*       &            &            & $-$*       &            &            & $-$*       &            &            & $-$*       &            & $+$*       &            &             \\

\hline
\multicolumn{2}{l|}{\textbf{RF}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            & $-$*       &            &            & $-$*       &            &            & $-$*       &            &            & $-$*       &            &            & $-$*       &             \\
&ip\_m        & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*        \\
&m            &            & $-$*       &            &            & $-$*       &            &            & $-$*       &            &            & $-$*       &            &            & $-$*       &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            & $-$*       & $-$*       &            &            & $-$*       &            &            & $-$*       &            &            & $-$*       &            &            & $-$*        \\
&ip\_m        & $+$*       &            & $-$*       &            &            & $-$*       &            &            & $-$*       &            &            & $-$*       &            &            & $-$*        \\
&m            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &             \\

\hline
\multicolumn{2}{l|}{\textbf{QDA}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            & $-$*       & $+$*       &            &            & $+$*       &            &            & $+$*       &            &            & $+$*       &            &            &             \\
&ip\_m        & $+$*       &            & $+$*       &            &            & $+$*       &            &            & $+$*       &            &            & $+$*       &            &            &             \\
&m            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            &            &            &             \\

\hline
\hline
\hline
\end{tabular}

  }
\end{table}

==> sections/gen-2-data/plots.tex <==


\begin{figure}[htbp]
\floatconts
  {fig:gen-2}
  {\caption{$\sigma = 2$: \textit{M} - dashed line,
  \textit{IP} - dash and dot line, \textit{IP\_M} - thin solid line.}}
  {%
    \subfigure[Visualization of 4 classes]{
    \label{fig:gen-2:dist-class}%
    \includeteximage{plots/gen-2-class-visualization-partial}
    }%
    \qquad
    \subfigure[Baseline error, $b\_err$]{\label{fig:gen-2:baseline-error}%
      \includeteximage{plots/gen-2-baseline-error}
      }
    \qquad
    \subfigure[$oneC$: SVM and DT]{\label{fig:gen-2:oneC-SVM-DT}%
      \includeteximage{plots/gen-2-oneC-0}
      %\includeteximage{plots/gen-2-dist-class}
      }
    \qquad
    \subfigure[$avgC$: SVM and DT]{\label{fig:gen-2:avgC-SVM-DT}%
      \includeteximage{plots/gen-2-avgC-0}
      }
    \qquad
    \subfigure[$oneC$: KNN and Ada]{\label{fig:gen-2:oneC-KNN-Ada}%
      \includeteximage{plots/gen-2-oneC-2}
      }
    \qquad
    \subfigure[$avgC$: KNN and Ada]{\label{fig:gen-2:avgC-KNN-Ada}%
      \includeteximage{plots/gen-2-avgC-2}
      }
    \qquad
    \subfigure[$oneC$: GNB and MPR]{\label{fig:gen-2:oneC-GNB-MPR}%
      \includeteximage{plots/gen-2-oneC-4}
      }
    \qquad
    \subfigure[$avgC$: GNB and MPR]{\label{fig:gen-2:avgC-GNB-MPR}%
      \includeteximage{plots/gen-2-avgC-4}
      }
    \qquad
    \subfigure[$oneC$: RF and QDA]{\label{fig:gen-2:oneC-RF-QDA}%
      \includeteximage{plots/gen-2-oneC-6}
      }
    \qquad
    \subfigure[$avgC$: RF and QDA]{\label{fig:gen-2:avgC-RF-QDA}%
      \includeteximage{plots/gen-2-avgC-6}
      }
  }
\end{figure}




==> sections/gen-2-data/table_threshold.tex <==
\begin{table}[htbp]
\scriptsize
 % The first argument is the label.
 % The caption goes in the second argument, and the table contents
 % go in the third argument.
\floatconts
  {tab:gen_2}%
  {\caption{Significance of results for $\sigma = 2$}}%
  {
\begin{tabular}{cl|lll|lll|lll|lll|lll}
             && \multicolumn{3}{c|}{$\epsilon=0.01$} & \multicolumn{3}{c|}{$\epsilon=0.05$} & \multicolumn{3}{c|}{$\epsilon=0.1$} & \multicolumn{3}{c|}{$\epsilon=0.15$} & \multicolumn{3}{c}{$\epsilon=0.2$} \\
\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*        \\
&ip\_m        & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*        \\
&m            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &             \\

\hline
\multicolumn{2}{l|}{\textbf{SVM}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*       &            &            & $-$*       & $+$*        \\
&ip\_m        & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*        \\
&m            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            &            & $-$*       &            & $-$*       & $-$*       &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*        \\
&ip\_m        & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*        \\
&m            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &             \\

\hline
\multicolumn{2}{l|}{\textbf{DT}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            & $-$        &            &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*        \\
&ip\_m        & $+$        &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*        \\
&m            &            & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            &            & $-$*       &            &            & $-$*        \\
&ip\_m        & $+$*       &            & $-$*       & $+$*       &            &            & $+$*       &            &            &            &            & $-$*       &            &            & $-$*        \\
&m            & $+$*       & $+$*       &            & $+$*       &            &            & $+$*       &            &            & $+$*       & $+$*       &            & $+$*       & $+$*       &             \\

\hline
\multicolumn{2}{l|}{\textbf{KNN}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            &            & $+$*       &            &            & $-$*        \\
&ip\_m        & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*       &            &            & $+$*       &            &            & $-$*        \\
&m            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $-$*       & $-$*       &            & $+$*       & $+$*       &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*        \\
&ip\_m        & $+$*       &            &            & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            &            & $+$*       &            & $-$*        \\
&m            & $+$*       &            &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       &            &            & $+$*       & $+$*       &             \\

\hline
\multicolumn{2}{l|}{\textbf{Ada}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       &            &            & $-$*       & $+$*       &            & $-$*       & $+$*        \\
&ip\_m        & $+$*       &            &            & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*        \\
&m            & $+$*       &            &            & $+$*       & $-$*       &            &            & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*        \\
&ip\_m        & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*        \\
&m            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &             \\

\hline
\multicolumn{2}{l|}{\textbf{GNB}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*       &            &            & $-$*       & $-$*       &            & $-$*       & $-$*        \\
&ip\_m        & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*        \\
&m            & $-$*       & $-$*       &            & $-$*       & $-$*       &            &            & $-$*       &            & $+$*       & $-$*       &            & $+$*       & $-$*       &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*        \\
&ip\_m        & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*        \\
&m            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &             \\

\hline
\multicolumn{2}{l|}{\textbf{MPR}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*        \\
&ip\_m        & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*        \\
&m            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*        \\
&ip\_m        & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            &            & $+$*       &            & $+$*        \\
&m            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       &            &            & $+$*       & $-$*       &             \\

\hline
\multicolumn{2}{l|}{\textbf{RF}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*        \\
&ip\_m        &            &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*        \\
&m            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*        \\
&ip\_m        & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*        \\
&m            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &             \\

\hline
\multicolumn{2}{l|}{\textbf{QDA}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*        \\
&ip\_m        & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*        \\
&m            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $+$*       & $-$*       &            & $+$*       & $-$*       &            & $+$*       & $-$*       &             \\

\hline
\hline
\hline
\end{tabular}

  }
\end{table}

==> sections/gen-5-data/plots.tex <==


\begin{figure}[htbp]
\floatconts
  {fig:gen-5}
  {\caption{$\sigma = 5$: \textit{M} - dashed line,
  \textit{IP} - dash and dot line, \textit{IP\_M} - thin solid line.}}
  {%
    \subfigure[Visualization of 4 classes]{
    \label{fig:gen-5:dist-class}%
    \includeteximage{plots/gen-5-class-visualization-partial}
    }%
    \qquad
    \subfigure[Baseline error, $b\_err$]{\label{fig:gen-5:baseline-error}%
      \includeteximage{plots/gen-5-baseline-error}
      }
    \qquad
    \subfigure[$oneC$: SVM and DT]{\label{fig:gen-5:oneC-SVM-DT}%
      \includeteximage{plots/gen-5-oneC-0}
      %\includeteximage{plots/gen-5-dist-class}
      }
    \qquad
    \subfigure[$avgC$: SVM and DT]{\label{fig:gen-5:avgC-SVM-DT}%
      \includeteximage{plots/gen-5-avgC-0}
      }
    \qquad
    \subfigure[$oneC$: KNN and Ada]{\label{fig:gen-5:oneC-KNN-Ada}%
      \includeteximage{plots/gen-5-oneC-2}
      }
    \qquad
    \subfigure[$avgC$: KNN and Ada]{\label{fig:gen-5:avgC-KNN-Ada}%
      \includeteximage{plots/gen-5-avgC-2}
      }
    \qquad
    \subfigure[$oneC$: GNB and MPR]{\label{fig:gen-5:oneC-GNB-MPR}%
      \includeteximage{plots/gen-5-oneC-4}
      }
    \qquad
    \subfigure[$avgC$: GNB and MPR]{\label{fig:gen-5:avgC-GNB-MPR}%
      \includeteximage{plots/gen-5-avgC-4}
      }
    \qquad
    \subfigure[$oneC$: RF and QDA]{\label{fig:gen-5:oneC-RF-QDA}%
      \includeteximage{plots/gen-5-oneC-6}
      }
    \qquad
    \subfigure[$avgC$: RF and QDA]{\label{fig:gen-5:avgC-RF-QDA}%
      \includeteximage{plots/gen-5-avgC-6}
      }
  }
\end{figure}




==> sections/gen-5-data/table_threshold.tex <==
\begin{table}[htbp]
\scriptsize
 % The first argument is the label.
 % The caption goes in the second argument, and the table contents
 % go in the third argument.
\floatconts
  {tab:gen_5}%
  {\caption{Significance of results for $\sigma = 5$}}%
  {
\begin{tabular}{cl|lll|lll|lll|lll|lll}
             && \multicolumn{3}{c|}{$\epsilon=0.01$} & \multicolumn{3}{c|}{$\epsilon=0.05$} & \multicolumn{3}{c|}{$\epsilon=0.1$} & \multicolumn{3}{c|}{$\epsilon=0.15$} & \multicolumn{3}{c}{$\epsilon=0.2$} \\
\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*        \\
&ip\_m        & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*        \\
&m            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &             \\

\hline
\multicolumn{2}{l|}{\textbf{SVM}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*        \\
&ip\_m        & $+$*       &            &            & $+$*       &            &            & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*        \\
&m            & $+$*       &            &            & $+$*       &            &            & $+$*       & $-$*       &            & $+$*       & $-$*       &            & $+$*       & $-$*       &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*        \\
&ip\_m        & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*        \\
&m            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &             \\

\hline
\multicolumn{2}{l|}{\textbf{DT}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            & $-$*       &            &            & $-$*       &            &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*        \\
&ip\_m        & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*        \\
&m            &            & $-$*       &            &            & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            &            & $-$*        \\
&ip\_m        & $+$*       &            & $-$*       & $+$*       &            &            & $+$*       &            &            & $+$*       &            & $-$*       &            &            & $-$*        \\
&m            & $+$*       & $+$*       &            & $+$*       &            &            & $+$*       &            &            & $+$*       & $+$*       &            & $+$*       & $+$*       &             \\

\hline
\multicolumn{2}{l|}{\textbf{KNN}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            &            & $+$*        \\
&ip\_m        & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*       &            &            & $+$*        \\
&m            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $-$*       & $-$*       &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*        \\
&ip\_m        & $+$*       &            &            & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*        \\
&m            & $+$*       &            &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &             \\

\hline
\multicolumn{2}{l|}{\textbf{Ada}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            & $-$*       & $-$*       &            & $-$*       &            &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*        \\
&ip\_m        & $+$*       &            &            & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*        \\
&m            & $+$*       &            &            &            & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*        \\
&ip\_m        & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*        \\
&m            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &             \\

\hline
\multicolumn{2}{l|}{\textbf{GNB}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            & $-$*       &            &            & $-$*       &            &            & $-$*       &            &            & $-$*       &            & $-$*       &             \\
&ip\_m        &            &            & $-$*       &            &            & $-$*       &            &            & $-$*       &            &            &            & $+$*       &            &             \\
&m            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       &            &            &            &            &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*        \\
&ip\_m        & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*        \\
&m            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &             \\

\hline
\multicolumn{2}{l|}{\textbf{MPR}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            & $-$*       &            &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*        \\
&ip\_m        & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*        \\
&m            &            & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*        \\
&ip\_m        & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*        \\
&m            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &             \\

\hline
\multicolumn{2}{l|}{\textbf{RF}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            &            &            & $-$*       &            &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*        \\
&ip\_m        &            &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*        \\
&m            &            & $-$*       &            &            & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*        \\
&ip\_m        & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*        \\
&m            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &             \\

\hline
\multicolumn{2}{l|}{\textbf{QDA}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            & $-$*       &            &            & $-$*       &            &            & $-$*       &            &            & $-$*       &            & $-$*       &             \\
&ip\_m        &            &            & $-$*       &            &            & $-$*       &            &            & $-$*       &            &            &            & $+$*       &            &             \\
&m            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       &            &            &            &            &             \\

\hline
\hline
\hline
\end{tabular}

  }
\end{table}

==> sections/tables/cool-table_threshold.tex <==
\begin{table}[htbp]
\scriptsize
 % The first argument is the label.
 % The caption goes in the second argument, and the table contents
 % go in the third argument.
\floatconts
  {tab:cool}%
  {\caption{cool dataset}}%
  {
\begin{tabular}{cl|lll|lll|lll|lll|lll}
             && \multicolumn{3}{c|}{$\epsilon=0.01$} & \multicolumn{3}{c|}{$\epsilon=0.05$} & \multicolumn{3}{c|}{$\epsilon=0.1$} & \multicolumn{3}{c|}{$\epsilon=0.15$} & \multicolumn{3}{c}{$\epsilon=0.2$} \\
\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            &            &            &            &            &            &            & $-$*       &            &            & $-$*       &            &            & $-$*        \\
&ip\_m        &            &            &            &            &            &            &            &            & $-$*       &            &            & $-$*       &            &            & $-$*        \\
&m            &            &            &            &            &            &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &             \\

\hline
\multicolumn{2}{l|}{\textbf{SVM}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            & $+$*       &            &            & $+$*       &            &            & $+$*       &            &            & $+$        &            &            &             \\
&ip\_m        &            &            & $+$*       &            &            & $+$*       &            &            & $+$*       &            &            & $+$        &            &            &             \\
&m            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$        & $-$        &            &            &            &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            & $-$        &            & $-$        & $-$*       &            &            & $-$*       &            &            &            &            &            &             \\
&ip\_m        &            &            & $-$        & $+$        &            & $-$*       &            &            & $-$        &            &            &            &            &            &             \\
&m            & $+$        & $+$        &            & $+$*       & $+$*       &            & $+$*       & $+$        &            &            &            &            &            &            &             \\

\hline
\multicolumn{2}{l|}{\textbf{DT}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            & $-$        &            &            & $+$*       &            &            & $+$*       &            &            &            &            &            &             \\
&ip\_m        &            &            & $-$        &            &            & $+$*       &            &            & $+$*       &            &            &            &            &            &             \\
&m            & $+$        & $+$        &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            &            &            &            &            &            &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            &            &            &            & $-$*       &            &            & $-$*       &            & $-$        & $-$*       &            &            & $-$         \\
&ip\_m        &            &            &            &            &            & $-$*       &            &            & $-$*       & $+$        &            & $-$*       &            &            & $-$         \\
&m            &            &            &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$        & $+$        &             \\

\hline
\multicolumn{2}{l|}{\textbf{KNN}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            &            &            &            &            &            &            &            &            &            & $-$*       &            &            &             \\
&ip\_m        &            &            &            &            &            &            &            &            &            &            &            & $-$*       &            &            &             \\
&m            &            &            &            &            &            &            &            &            &            & $+$*       & $+$*       &            &            &            &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            &            &            &            &            &            &            & $+$*       &            &            &            &            &            & $-$*        \\
&ip\_m        &            &            &            &            &            &            &            &            & $+$*       &            &            &            &            &            & $-$         \\
&m            &            &            &            &            &            &            & $-$*       & $-$*       &            &            &            &            & $+$*       & $+$        &             \\

\hline
\multicolumn{2}{l|}{\textbf{Ada}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            & $+$*       &            &            & $+$*       &            &            & $+$*       &            &            & $+$*       &            &            & $+$*        \\
&ip\_m        &            &            & $+$*       &            &            & $+$*       &            &            & $+$*       &            &            & $+$*       &            &            & $+$*        \\
&m            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            & $-$*       &            & $-$*       & $-$*       &            & $-$        & $-$*       &            &            & $-$*       &            &            & $-$*        \\
&ip\_m        &            &            & $-$*       & $+$*       &            & $-$*       & $+$        &            & $-$*       &            &            & $-$*       &            &            & $-$*        \\
&m            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &             \\

\hline
\multicolumn{2}{l|}{\textbf{GNB}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            &            &            & $-$        & $-$*       &            & $-$        & $-$        &            &            & $+$        &            &            & $+$*        \\
&ip\_m        &            &            &            & $+$        &            & $-$*       & $+$        &            & $-$        &            &            & $+$        &            &            & $+$*        \\
&m            &            &            &            & $+$*       & $+$*       &            & $+$        & $+$        &            & $-$        & $-$        &            & $-$*       & $-$*       &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*        \\
&ip\_m        &            &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*        \\
&m            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &             \\

\hline
\multicolumn{2}{l|}{\textbf{MPR}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            & $+$*       &            &            & $+$*       &            &            & $+$*       &            &            & $+$*       &            & $-$*       & $+$*        \\
&ip\_m        &            &            & $+$*       &            &            & $+$*       &            &            & $+$*       &            &            & $+$*       & $+$*       &            & $+$*        \\
&m            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$        & $-$*        \\
&ip\_m        &            &            & $-$*       & $+$*       &            & $-$        & $+$*       &            & $-$        & $+$*       &            &            & $+$        &            & $-$         \\
&m            & $+$*       & $+$*       &            & $+$*       & $+$        &            & $+$*       & $+$        &            & $+$*       &            &            & $+$*       & $+$        &             \\

\hline
\multicolumn{2}{l|}{\textbf{RF}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            & $+$*       &            &            & $+$*       &            & $-$*       &            &            & $-$*       &            &            &            &             \\
&ip\_m        &            &            & $+$*       &            &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       &            &            &             \\
&m            & $-$*       & $-$*       &            & $-$*       & $-$*       &            &            & $-$*       &            &            & $-$*       &            &            &            &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&m            &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\

\hline
\multicolumn{2}{l|}{\textbf{QDA}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&m            &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\

\hline
\hline
\hline
\end{tabular}

  }
\end{table}

==> sections/tables/heat-table_threshold.tex <==
\begin{table}[htbp]
\scriptsize
 % The first argument is the label.
 % The caption goes in the second argument, and the table contents
 % go in the third argument.
\floatconts
  {tab:heat}%
  {\caption{heat dataset}}%
  {
\begin{tabular}{cl|lll|lll|lll|lll|lll}
             && \multicolumn{3}{c|}{$\epsilon=0.01$} & \multicolumn{3}{c|}{$\epsilon=0.05$} & \multicolumn{3}{c|}{$\epsilon=0.1$} & \multicolumn{3}{c|}{$\epsilon=0.15$} & \multicolumn{3}{c}{$\epsilon=0.2$} \\
\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*        \\
&ip\_m        &            &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*        \\
&m            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &             \\

\hline
\multicolumn{2}{l|}{\textbf{SVM}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            & $+$*       &            & $-$        & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            &            & $+$*        \\
&ip\_m        &            &            & $+$*       & $+$        &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       &            &            & $+$*        \\
&m            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            &            &            &            & $-$        &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            &            &            &            & $-$        &            &            &            &            &            &            &            &            &             \\
&m            &            &            &            & $+$        & $+$        &            &            &            &            &            &            &            &            &            &             \\

\hline
\multicolumn{2}{l|}{\textbf{DT}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            & $+$        &            &            & $+$*       &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            & $+$        &            &            & $+$*       &            &            &            &            &            &            &            &            &             \\
&m            & $-$        & $-$        &            & $-$*       & $-$*       &            &            &            &            &            &            &            &            &            &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            & $-$*       &            &            & $-$*       &            & $-$        & $-$*       &            & $-$        & $-$*       &            &            & $-$*        \\
&ip\_m        &            &            & $-$*       &            &            & $-$*       & $+$        &            & $-$*       & $+$        &            & $-$*       &            &            & $-$*        \\
&m            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &             \\

\hline
\multicolumn{2}{l|}{\textbf{KNN}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            & $-$*       &            &            & $+$*       &            &            & $-$*       &            &            & $-$*       &            &            & $-$*        \\
&ip\_m        &            &            & $-$*       &            &            & $+$*       &            &            & $-$*       &            &            & $-$*       &            &            & $-$*        \\
&m            & $+$*       & $+$*       &            & $-$*       & $-$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            &            &            &            &            &            &            &            &            &            & $-$        &            &            & $-$*        \\
&ip\_m        &            &            &            &            &            &            &            &            &            &            &            & $-$        &            &            & $-$*        \\
&m            &            &            &            &            &            &            &            &            &            & $+$        & $+$        &            & $+$*       & $+$*       &             \\

\hline
\multicolumn{2}{l|}{\textbf{Ada}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            & $+$*       &            &            & $+$        &            &            & $+$*       &            &            & $+$*       &            &            & $+$*        \\
&ip\_m        &            &            & $+$*       &            &            & $+$        &            &            & $+$*       &            &            & $+$*       &            &            & $+$*        \\
&m            & $-$*       & $-$*       &            & $-$        & $-$        &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            & $-$*       &            &            & $-$*       &            &            & $-$        &            &            & $-$*       &            &            & $-$*        \\
&ip\_m        &            &            & $-$*       &            &            & $-$*       &            &            & $-$        &            &            & $-$*       &            &            & $-$*        \\
&m            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$        & $+$        &            & $+$*       & $+$*       &            & $+$*       & $+$*       &             \\

\hline
\multicolumn{2}{l|}{\textbf{GNB}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            & $-$*       &            &            & $+$*       &            &            & $+$*       &            &            & $+$*       &            &            & $+$*        \\
&ip\_m        &            &            & $-$*       &            &            & $+$*       &            &            & $+$*       &            &            & $+$*       &            &            & $+$*        \\
&m            & $+$*       & $+$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*        \\
&ip\_m        &            &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*        \\
&m            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &             \\

\hline
\multicolumn{2}{l|}{\textbf{MPR}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*       &            & $-$*       & $+$*        \\
&ip\_m        &            &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*        \\
&m            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*       &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            & $-$*       &            & $-$*       & $-$        &            & $-$*       & $-$*       &            & $-$*       & $-$*       &            & $-$*       & $-$*        \\
&ip\_m        &            &            & $-$*       & $+$*       &            & $+$*       & $+$*       &            &            & $+$*       &            & $-$*       & $+$*       &            & $-$*        \\
&m            & $+$*       & $+$*       &            & $+$        & $-$*       &            & $+$*       &            &            & $+$*       & $+$*       &            & $+$*       & $+$*       &             \\

\hline
\multicolumn{2}{l|}{\textbf{RF}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            & $+$*       &            & $-$*       & $+$*       &            & $-$*       &            &            & $-$*       &            &            &            &             \\
&ip\_m        &            &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       & $+$*       &            & $+$*       &            &            &             \\
&m            & $-$*       & $-$*       &            & $-$*       & $-$*       &            &            & $-$*       &            &            & $-$*       &            &            &            &             \\

\hline
\hline
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$oneC$}}&ip           &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&m            &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\

\hline
\multicolumn{2}{l|}{\textbf{QDA}} & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m          & ip         & ip\_m      & m           \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{$avgC$}}&ip           &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&ip\_m        &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\
&m            &            &            &            &            &            &            &            &            &            &            &            &            &            &            &             \\

\hline
\hline
\hline
\end{tabular}

  }
\end{table}
